Continuously Optimizing Radar Placement with Model Predictive Path Integrals

Continuously optimizing sensor placement is essential for precise target localization in various military and civilian applications. While information theory has shown promise in optimizing sensor placement, many studies oversimplify sensor measurement models or neglect dynamic constraints of mobile sensors. To address these challenges, we employ a range measurement model that incorporates radar parameters and radar-target distance, coupled with Model Predictive Path Integral (MPPI) control to manage complex environmental obstacles and dynamic constraints. We compare the proposed approach against stationary radars or simplified range measurement models based on the root mean squared error (RMSE) of the Cubature Kalman Filter (CKF) estimator for the targets' state. Additionally, we visualize the evolving geometry of radars and targets over time, highlighting areas of highest measurement information gain, demonstrating the strengths of the approach. The proposed strategy outperforms stationary radars and simplified range measurement models in target localization, achieving a 38-74% reduction in mean RMSE and a 33-79% reduction in the upper tail of the 90% Highest Density Interval (HDI) over 500 Monte Carl (MC) trials across all time steps. Code will be made publicly available upon acceptance.

==> ieeecopyright.tex <==
{\onecolumn
\noindent \textbf{\large IEEE Copyright Notice} \\ \\
© 2024 IEEE. Personal use of this material is permitted. Permission from IEEE must be obtained for all other uses, in any current or future media, including reprinting/republishing this material for advertising or promotional purposes, creating new collective works, for resale or redistribution to servers or lists, or reuse of any copyrighted component of this work in other works \\ \\

\noindent Submitted for review to: IEEE Journal - Transactions on Aerospace and Electronics - 2024
}

==> introduction/introduction_draft1.tex <==
\section{INTRODUCTION}
\label{sec:intro}
In military operations, a common scenario involves the deployment of moving radars tasked with tracking multiple aerial targets in dynamic environments. This scenario typically unfolds on a battlefield where military forces face threats from enemy aircraft or drones \cite{grant2010radar}. Radars, often mounted on vehicles or strategically positioned, play a critical role in providing continuous airspace surveillance \cite{butowsky1994opana}. Ideally, the radars would dynamically adjust their positions to maintain optimal coverage while avoiding detection and potential threats. Thus, effective coordination between radars and ground forces is imperative for successful target localization.

Target localization, which is the estimation of target position and/or velocity from noisy radar-based measurements, presents a challenge across both military and civilian applications, including intelligent transportation, navigation, defense surveillance, and emergency rescue \cite{ding2023radar,venkatasubramanian2023datadriven}. 
The accuracy of target localization in these applications is significantly influenced by the relative radar-target geometry, which underscores the importance of comprehending and optimizing this relationship \cite{godrich2010target,sadeghi2021target}.

Many authors integrate radar-target geometry into an objective function. This is achieved by evaluating the performance of static-target localization using the \gls{pcrlb}, which is the inverse of the \gls{pfim}, of the estimator variance based on radar measurements \cite{tichavsky1998posterior,bishop2010optimality,moreno2011optimal,zhao2002information}. Thus, the optimal radar placement is determined by maximizing the determinant/trace of the \gls{pfim} (D-optimality/A-Optimality \cite{jones2021optimal}) with respect to the radar position, which in turn minimizes the uncertainty ellipse of the estimator. Given that the mean-squared error of an estimator is decomposed into the bias and variance of the estimator, it is evident that the above statement is equivalent to minimizing the mean squared error of an estimator \cite{bishop2006pattern}.

However, as static targets become dynamic, the optimal radar configuration at one time step may no longer remain optimal at the next time step. Historically, there have been two main approaches to optimal radar placement for target localization of dynamic targets: 1) move the radars to track dynamic targets while preserving an optimal radar-target localization geometry \cite{martinez2006optimal}
and 2) "spray" radars over a large area to ensure high spatial coverage and multiplicity, then choose which radars to employ for sensing \cite{zhao2002information}. This paper primarily focuses on approach 1, which involves computing the \gls{pfim} for multiple future time steps based on an estimation of the target's trajectory. 


Consequentially, rather than directly optimizing the radar's position at a specific time step, as in the static target-localization problem, the optimal radar position is indirectly determined by optimizing the control inputs to the radar kinematic model \cite{martinez2006optimal,cai2021non,crasta2018multiple}. This problem is typically solved with a \gls{mpc}, which minimizes the predicted D-optimality of the \gls{pfim} over a finite, receding horizon, while taking into account the radar dynamic constraints (and system constraints) \cite{mpc_overview,mpc_matlab}.


==> introduction/introduction_draft2.tex <==
\section{INTRODUCTION}
\label{sec:intro}


The deployment of automatic mobile sensors to detect and localize numerous targets in dynamic environments is a highly active research field in both civilian and military domains \cite{grant2010radar,kumar2021recent}. These applications encompass intelligent transportation, navigation, defense surveillance, and emergency rescue \cite{ding2023radar,venkatasubramanian2023datadriven}. Target localization involves estimating target position and/or velocity from noisy sensor-based measurements. In military applications, radars have been ubiquitous for target localization since World War II, where effective radar positioning in an environment has been pivotal for mission success \cite{butowsky1994opana}. Ideally, sensors would dynamically adjust their positions to ensure optimal coverage of enemy combatants while reducing the risk of detection and threats, thereby potentially enhancing mission success. These "cognitive radars" \cite{gurbuz2019overview} would not only improve coverage but also signifies a notable evolution in modern warfare tactics. Furthermore, the accuracy of target localization within these realms is significantly affected by factors such as the sensing technology employed and the relative radar-target geometry, making understanding and optimizing these relationships paramount \cite{godrich2010target,sadeghi2021target,sensingtech}.

While a plethora of sensing technologies are explored in the multi-target tracking and sensor placement literature, including cameras \cite{yoon2009autonomous}, ultrasonic sensors \cite{juan2021object,ray2002genetic}, \gls{li} \cite{9810346}, and acoustic range sensors \cite{crasta2018multiple}, our focus lies on radar in the \gls{uhf}. Radar systems are ubiquitous in target detection and localization applications due to their long-range detection capability, adeptness in penetrating obstacles such as atmospheric conditions, and versatility in capturing detailed target features \cite{richards2010principles}.

Moreover, many authors incorporate radar-target geometry into an objective function by assessing target localization performance using the \gls{pcrlb}, derived from the \gls{pfim}, which evaluates estimator variance based on radar measurements \cite{tichavsky1998posterior,bishop2010optimality,moreno2011optimal,zhao2002information}. 
However, many of these studies optimizing sensor placement typically rely on a simplified measurement model, such as range measurement with a constant covariance matrix, which overlooks the effects of signal path attenuation \cite{crasta2018multiple,cai2021non,hung2020range,9812315}. Our approach, inspired by \cite{godrich2010target}, utilizes an \gls{fim} where the covariance matrix of the range measurement is directly proportional to the receive power at the radar after signal path attenuation.

In scenarios where radars have mobile capabilities and the target is dynamic, the optimal radar-target geometry at one time step may significantly differ from future time steps. Consequently, many studies focusing on dynamic-sensor-(static/dynamic)-target configurations employ a \gls{mpc} objective for optimizing the control inputs of mobile radar dynamics \cite{khan2022design,uluskan2020noncausal,chu2020trajectory,sture2020trajectory,hung2020range} over a finite horizon \cite{mpc_matlab}, incorporating the \gls{pcrlb}/\gls{pfim} in the instantaneous cost function. However, optimizing \gls{mpc} for nonlinear functions, typical when involving \gls{pcrlb}/\gls{pfim}, may be computationally and time-intensive with deterministic optimization algorithms that require differentiable, continuous, or linearized objectives. 
Therefore, we employ \gls{mppi} control to estimate the optimal control inputs to the radars, leveraging its advantages in directly accounting for noise characteristics and dynamics of the vehicles during optimization \cite{williams2018information}. 
\gls{mppi} control enables defining the instantaneous cost function with fewer restrictions, such as smoothness, and facilitates highly parallel computation \cite{mppi_advantages} for real-time control applications.

To address these issues, this paper develops a pipeline utilizing state-of-the-art techniques for continuous optimal radar placement by optimizing radar trajectories with \gls{mppi} control. Here, we incorporate signal path attenuation on the received radar signal in the computation of the \gls{pfim}. Additionally, by employing \gls{mppi} for optimal control, we gain more flexibility for future work, including handling more nonlinear, discontinuous, and non-differentiable objectives.

The paper is structured  as follows: \cref{sec:related_works} describes the current literature; \cref{sec:preliminaries} describes the simulation assumptions and notation; \textcolor{red}{tbd}

==> introduction/introduction_draft3.tex <==
\section{INTRODUCTION}
\label{sec:intro}

Deploying a fleet of autonomous mobile sensors to estimate the positions and velocities of targets over time is an important research problem, with applications in transportation, navigation, defense, surveillance, and emergency rescue~\cite{ding2023radar,venkatasubramanian2023datadriven,grant2010radar,kumar2021recent}, exemplified in \cref{appfig:conops}. This problem involves multiple challenges, including predicting expected sensor information gain without exact target or measurement data, adapting mobile sensors planned trajectories to dynamic environmental and target changes, and selecting suitable sensor models and modalities. We will discuss these challenges in the following paragraphs.

The multi-target tracking and sensor placement literature has explored various sensing modalities, including cameras \cite{yoon2009autonomous}, ultrasonic sensors \cite{juan2021object,ray2002genetic}, \gls{li} \cite{9810346}, acoustic range sensors \cite{crasta2018multiple}, and radar-based techniques dating back to World War II.
This paper focuses on tracking with radar in the \gls{uhf} (particularly ``cognitive radars'' \cite{gurbuz2019overview}), due to the long-range detection capability, ability to penetrate atmospheric obstacles, and versatility in capturing detailed target features \cite{richards2010principles}.
% Our approach consists of algorithm estimating target states from noisy radar data, while simultaneously controlling the position of the radars to improve the target estimates without

% This target localization problem 
% has long relied on radars in military operations, dating back to World War II, where radar positioning was crucial for mission success \cite{butowsky1994opana}. Ideally, radars would dynamically adjust positions to optimize coverage of enemy combatants while minimizing detection risks, thereby increasing the likelihood of mission success. That being said, the accuracy of target localization hinges on factors like sensing technology and sensor-target geometry, highlighting the importance of understanding and optimizing these relationships \cite{godrich2010target,sadeghi2021target,sensingtech}.
% Radars are ubiquitous in target detection and localization 

% need to relate radar/target geometry to target localization performance -> use PCRLB/PFIM -> most people only do this with overly simple sensor model
A key challenge in radar-based target tracking is in incorporating realistic sensor models into the information metrics used for controlling the sensors.
In particular, most existing control strategies for this problem use the \gls{pfim} \cite{tichavsky1998posterior} (inverse of the \gls{pcrlb}) to quantify the relationship between radar-target geometry and target localization performance \cite{bishop2010optimality,moreno2011optimal,zhao2002information}. However, studies optimizing sensor placement often oversimplify by using a constant covariance matrix for range measurements, neglecting signal path attenuation effects \cite{kumar2021recent}.  The approach in \cite{kumar2021recent} focuses on optimizing the angle subtended between the radars and targets but does not encourage the mobile radars to move closer to the target. In \cite{godrich2010target}, the authors provide the error covariance matrix of a \gls{blue} estimator for the range measurement using a first-order Taylor Series approximation of a \gls{ddr} measurement model, which yields the \gls{fim}. Similarly, we calculate the \gls{fim} for the the \gls{ddr} measurement model from \cite{godrich2010target}, where the covariance matrix of the range measurement is directly proportional to the received power at the radar after signal path attenuation, but we do not apply a first-order Taylor Series approximation to the \gls{ddr} measurement model. This strategy encourages mobile radars to move closer to the targets, thereby increasing the \gls{snr} and improving radar range measurements.

% dynamic environment -> need mpc -> hard to solve because of nonlinear FIM objective -> propose to use mppi
Another major challenge in scenarios with moving targets and movable radars is that the optimal radar-target geometry may change substantially over time.
Consequently, many studies use \gls{mpc} \cite{mpc_matlab} for choosing the control inputs of mobile sensors over a finite horizon in response to uncertain target state estimates \cite{khan2022design,uluskan2020noncausal,chu2020trajectory,sture2020trajectory,hung2020range}. However, natural choices for the \gls{mpc} objective in this problem, such as minimizing/maximizing the  D-optimality of \gls{pcrlb}/\gls{pfim}, lead to challenging nonlinear optimization problems that are computationally prohibitive to solve exactly.
To address this issue, we instead utilize \gls{mppi} to approximate the optimal control inputs for the mobile radars, enabling the handling of discontinuous, non-smooth objectives through highly parallelized computation for real-time control \cite{mppi_advantages,williams2018information}.
% Typically, the number of samples needed to estimate the parameters of the \gls{pdf} with a desired level of accuracy grows exponentially with the dimensionality of the parameters, known as the curse of dimensionality \cite{bishop2006pattern}.
However, as the number of agents, planning horizon, and the actuation space increases, parameter estimation, particularly for the covariance, requires an exponentially growing number of samples. To mitigate this issue and reduce the number of proposal distribution updates and trajectory samples needed in the high-dimensional control space, we integrate advanced \gls{ais} techniques, such as cross-entropy weighting with covariance shrinkage \cite{asmar2023model}, to prevent overfitting of the sample covariance matrix.


% optimizing \gls{mpc} objectives for nonlinear functions, particularly those involving \gls{pcrlb}/\gls{pfim}, may be computationally intensive and impose restrictive assumptions. Thus, 

This paper introduces a improved pipeline for continuously optimizing radar placement, aiming to overcome the previously mentioned challenges. We derived objective functions using the \glspl{fim} that incorporate signal path attenuation and optimize these functions with respect to radar control inputs using \gls{mppi} control. Crucially, \gls{mppi} control provides increased flexibility for real-time optimization of nonlinear, discontinuous, and non-differentiable objectives in research, including future enhancements to signal measurement models and occupancy grid maps. Results from over 500 \gls{mc} trials across various simulation scenarios empirically show that our approach achieves lower \gls{rmse} compared to stationary radars and state estimators using simplified range measurement models, with reduced variance across \gls{mc} trials. 

The paper is structured as follows: \cref{sec:related_works} describes the current literature; \cref{sec:preliminaries} describes the simulation assumptions and notation; \cref{sec:radar_signal_model} describes the radar signal model and \gls{ddr} measurement model; \cref{sec:process_modeling} formulates the targets' state-space model and the radars' kinematic model; \cref{sec:fim_definition} derives the \gls{fim} which accounts for the radar signal attenuation; \cref{sec:mpc_objective} formulates our objective function based on the derived \glspl{fim} and outlines our \gls{mppi} controller, and \cref{sec:experiment} discusses the results of the proposed approach for three simulation scenarios.

==> methodology/methodology_draft1.tex <==
\section{Radar Signal Model}
\label{sec:radar_signal_model}
We assume there are $N$ radars transmitting orthogonal Narrowband signals to track $M$ targets as in \cite{godrich2010target}, where the received signal at radar $N$ is

\begin{align}
    r^{n}(t) &= \sum_{m=1}^M \zeta e^{-j2\pi f_c \tau^{nm}} s^m(t-\tau^{nm}) + \epsilon_{a}^n(t) \label{eqn:return_signal} \\
    \tau^{nm} &= \frac{2 \lVert \chi^{R_n}_{xyz} - \chi^{T_m}_{xyz} \rVert} {c} 
\end{align}

and the set of lowpass equivalent signals are $s(t)$ such that
\begin{align}
    \int_T s^i(t) s^j(t) = \begin{cases}
        0 & i\neq j \\
        1 & i=j
    \end{cases} dt
\end{align} 
The return signal noise $\epsilon_{a}(t)$ is circularly symmetric, zero-mean, complex Gaussian noise with autocorrelationn function $\sigma_a^2 \delta (\tau)$. We define $\zeta$ as the complex amplitude of the return signal, where $|\zeta|^2$ is the radar power return specified by the radar equation \cite{barton2013radar}:
\begin{align}
    |\zeta|^2 = P_r = \frac{P_t G_t G_r \lambda^2 \Xi}{(4\pi)^3 \lVert \chi^{R}_{xyz} - \chi^{T}_{xyz} \rVert ^4 L}
\end{align}
where $P_r$ is the received power $[W]$ at the radar, $P_t$ is the transmit power $[W]$ of the radar, $G_t$ and $G_r$ are the transmit and receive gains respectively, L is the general loss  factor, $\Xi$ is  the radar cross section $[m^2]$, and $\lambda$ is the carrier frequency wavelength $[m]$.

By maximizing the match filter as a function of time delay $\tau^{nm}$ and using second-order Taylor series expansion around $\tau^{nm}$, it is shown that the time delay between radar $n$ and target $m$ is distributed as Gaussian with  a variance that is parameterized by the radar-target geometry \cite{godrich2010target}
\begin{align}
    z^{nm} &= \tau^{nm} + \epsilon_z^{nm} \label{eqn:tod_measurement}\\
    \epsilon_z^{nm} &\sim \mathcal{N}\left(0,\frac{\sigma_a^2}{8\pi^2 f_c^2 |\zeta^{nm}|^2} \right) 
\end{align}

The density over radar-target paired range measurements is obtained by multiplying \cref{eqn:tod_measurement} by $c$ on both the left-hand side (LHS) and the right-hand side (RHS):

\begin{align}
z^{nm} \sim  \mathcal{N}\left(2 \lVert \chi^{R_n}_{xyz} - \chi^{T_m}_{xyz} \rVert \; , \; \frac{c^2 \sigma_a^2}{8\pi^2 f_c^2 |\zeta^{nm}|^2} \right) \label{eqn:range_measurement}
\end{align}

We denote all the radar parameters, signal parameters, and noise parameters as a constant $K=\frac{c^2 \sigma_a^2 (4\pi)^3 L}{P_t G_t G_r \lambda ^2 \Xi 8\pi^2 f_c^2} $. For brevity, we define shorthand notation  as 
$h^{nm} = 2 \lVert \chi^{R_n}_{xyz} - \chi^{T_m}_{xyz} \rVert $ and $\sigma_z^{nm} = \frac{c^2 \sigma_a^2}{8\pi^2 f_c^2 |\zeta^{nm}|^2}$.

Analysis  on optimal  radar placement when the covariance matrix of the range measurement is parameterized by the radar-target geometry has been studied in other works \cite{moreno2011optimal,yan2017exact,he2015generalized}, but for stationary targets and radars. 

Next, we describe the target kinematic models, enabling us to define the targets conditional transition probability.


\section{Process Modeling}
We describe the kinematic model of a target to finalize the probabilistic state space model for the concatenated state of all the targets, encompassing both a conditional transition probability and a conditional measurement probability.

\subsection{Target Constant Velocity Model}
Following \cite{baisa2020derivation}, we define the assumed target kinematic model for a single target undergoing constant velocity motion with acceleration noise, which specifies the conditional transition probability of a single target as:

\begin{align*}
\chi^T_{k+1} &= A\chi_k^T + \epsilon_Q \label{eqn:dynamics_single_target} \\
\end{align*}
where 
\begin{align*}
    A_{\text{single}} &= \begin{bmatrix}
        1 & 0 & 0 & \Delta t & 0 & 0 \\ 
        0 & 1 & 0 & 0 & \Delta t & 0 \\ 
        0 & 0 & 1 & 0 & 0 & \Delta t \\ 
        0 & 0 & 0 & 1 & 0 & 0 \\
        0 & 0 & 0 & 0 & 1 & 0 \\
        0 & 0 & 0 & 0 & 0 & 1 \\
    \end{bmatrix} \\ 
     W_{\text{single}} &= \begin{bmatrix}
        \frac{\Delta t^4}{4} & 0 & 0 & \frac{\Delta t^3}{2} & 0 & 0 \\ 
        0 & \frac{\Delta t^4}{4} & 0 & 0 & \frac{\Delta t^3}{2} & 0 \\ 
        0 & 0 & \frac{\Delta t^4}{4} & 0 & 0 & \frac{\Delta t^3}{2}\\ 
        \frac{\Delta t^3}{2} & 0 & 0 & \Delta t^2 & 0 & 0 \\
        0 & \frac{\Delta t^3}{2} & 0 & 0 & \Delta t^2 & 0 \\
        0 & 0 & \frac{\Delta t^3}{2} & 0 & 0 & \Delta t^2\\
    \end{bmatrix} \times \sigma_W^2
\end{align*}

Thus, the conditional transition probability for the state-space is defined as
\begin{align}
    A &= (I_{MM} \otimes A_{\text{single}}) \\
    W &= (I_{MM} \otimes W_{\text{single}}) \\
     \chi^{T_{1:M}}_{k+1} &= A \times \chi^{T_{1:M}}_k + \epsilon_{W} \label{eqn:transition_model} 
\end{align}

Similarly, the measurements of all radar-target pairs may be concatenated for the conditional measurement probability (based on \cref{eqn:range_measurement}):

\begin{align}
\mathbf{z}^{T_{1:M}} &= \begin{bmatrix}
h^{11} & \ldots & h^{1M} \\
h^{21} & \ldots & h^{2M} \\
\vdots & \ddots & \vdots \\
h^{N1} & \ldots & h^{NM} \\
\end{bmatrix} +  \begin{bmatrix}
\sigma_z^{11} & \ldots & \sigma_z^{1M} \\
\sigma_z^{21}  & \ldots & \sigma_z^{2M}  \\
\vdots & \ddots & \vdots \\
\sigma_z^{NM} & \ldots & \sigma_z^{nM}  \\
\end{bmatrix} \odot \epsilon_\mathbf{z} \label{eqn:measurement_prob} \\
\mathbf{z}^{T_{1:M}} &= \mathbf{H(\chi^{T_{1:M}}_{xyz}}) + W \odot \sigma_\mathbf{z}
\end{align}

and therefore the final state-space for the targets is 

\begin{align}
     \chi^{T_{1:M}}_{k+1} &= A \times \chi^{T_{1:M}}_k + \epsilon_{Q} \label{eqn:state_space_tran} \\
    \mathbf{z}^{T_{1:M}}_{k+1} &= \mathbf{H}\left((\chi^{T_{1:M}}_{xyz})_{k+1}\right) + W \odot \sigma_\mathbf{z} \label{eqn:state_space_meas} 
\end{align}

\textcolor{red}{Need to clean up above equations}

Since our focus is on non-stationary targets and radars, it's important to describe a simple kinematic model for the radars to ensure that their motion follows specific constraints.

\subsection{Radar Second Order Unicycle Model}

We use the Euler discretization of the Unicycle continuous dynamic model with heading acceleration and angular acceleration control inputs $u = [u_{a},u_{\dot{\omega}}]^T$:

% x_{k+1} &= x_{k} + \dot{x}_k \cos{\theta_k} \Delta t + \frac{1}{2} (u_{a})_k \cos{\theta_k} \Delta t^2  \\
% y_{k+1} &= y_{k} + \dot{y}_k \sin{\theta_k} \Delta t + \frac{1}{2} 
% (u_{a})_k \sin{\theta_k} \Delta t^2 \\
% z_{k+1} &= z_{k} \\
% \theta_{k+1} &= \theta_{k} + \omega_k \Delta t + \frac{1}{2} u_{\dot{\omega}_k} \Delta t^2 \\
% v_{k+1} &= v_k + (u_{a})_k \Delta t \\
% \omega_{k+1} &= \omega_{k} + (u_{\dot{\omega}})_k \Delta t \\

\begin{equation}
\begin{aligned}
    \begin{bmatrix}
        x_{k+1} \\
        y_{k+1} \\
        z_{k+1} \\
        \theta_{k+1} \\
        v_{k+1} \\ 
        \omega_{k+1}
    \end{bmatrix} &=
    \begin{bmatrix}
        1 &  0 & 0 & 0 & \cos \theta_k \Delta t & 0 \\
        0 & 1 & 0 & 0 & \sin \theta_k \Delta t & 0\\
        0 & 0 & 1 & 0 & 0 & 0 \\
        0 & 0 & 0 & 1 & 0 & \Delta t  \\
         0 & 0 & 0 & 0 & 1 & 0  \\
        0 & 0 & 0 & 0 & 0 & 1
    \end{bmatrix} 
        \begin{bmatrix}
        x_{k} \\
        y_{k} \\
        z_{k} \\
        \theta_{k} \\
        v_{k} \\
        \omega_{k}
    \end{bmatrix} +  \\ 
    & \begin{bmatrix}
     \frac{1}{2} \cos \theta_k \Delta t^2 & 0 \\
     \frac{1}{2} \sin \theta_k \Delta t^2 & 0 \\
    0  & 0  \\
    0  & \frac{1}{2} \Delta t^2 \\
    \Delta t & 0\\
        0 & \Delta t 
    \end{bmatrix} u_k \\
    \chi^{R}_{k+1} &= \chi^{R}_k + G_k(\chi^{R}_k,u_k)
\end{aligned}
        \label{eqn:radar_kinematics}
\end{equation}

where we constrain the velocity, angular velocity, and control inputs
\begin{equation}
\begin{aligned}
\begin{split}
\underbar{$u$}_a \leq u_{a_k} &\leq \bar{u}_a \; \forall k \\
\underbar{$u$}_{\dot{\omega}} \leq u_{\dot{\omega}_k} &\leq \bar{u}_{\dot{\omega}} \; \forall k  \\
\end{split} \quad
\begin{split}
\underbar{$v$} \leq v_k &\leq \bar{v} \; \forall k \\
\underbar{ $\omega$ } \leq \omega_k &\leq \bar{ \omega } \; \forall k
\end{split}
\end{aligned}
\label{eqn:radar_kinematics_constrained}
\end{equation}



The next section derives the \gls{sfim} for the targets' positions based on the radar-target measurement model \cref{eqn:range_measurement,eqn:measurement_prob} and the  radar position parameterized by \cref{eqn:radar_kinematics,eqn:radar_kinematics_constrained}.

\section{Fisher Information Matrix}
\label{sec:fim_definition}

The \gls{sfim} measures the amount of information that an observable random variable $z$ (range measurements) carries about an unknown parameter $\theta$ (targets' states) \cite{tichavsky1998posterior,kay1993fundamentals}:

\begin{align}
    J_D(\theta) = E\left[\left( \nabla_{\theta} \log f\left(z|\theta \right) \right) \left( \nabla_{\theta} \log f\left(z|\theta \right) \right)^T\right]
\end{align}

Under the assumption of independence, the likelihood of the range measurements in \cref{eqn:measurement_prob} is represented as:
\begin{align}
    f(\mathbf{z}^{T_{1:M}}|\chi^{T_{1:M}}_{xyz} ; \chi^{R_{1:N}}_{xyz}) &= \prod_{n=1}^{N} \prod_{m=1}^{M} f(z^{nm} | \chi^{T_m}_{xyz} ; \chi^{R_n}_{xyz})
\end{align}

and the log likelihood is 
\begin{align}
    \log  f(\mathbf{z}^{T_{1:M}}|\chi^{T_{1:M}}_{xyz} ; \chi^{R_{1:N}}_{xyz}) &= \sum_{n=1}^{N} \sum_{m=1}^{M} \log f(z^{nm} | \chi^{T_m}_{xyz} ; \chi^{R_n}_{xyz}) 
\end{align}

Given that the measurement follows a Gaussian density, where the mean and covariance are parameterized by the targets' positions, we can utilize the property: 

\begin{align}
    \mathbf{z}^{T_{1:M}} &\sim \mathcal{N}(\mu(\theta),\Sigma(\theta)) \\
    (J_{D})_{\theta_i,\theta_j} &= \frac{\partial \mu^T}{\partial \theta_i} \Sigma^{-1} \frac{\partial \mu}{\partial \theta_j} + \frac{1}{2} Tr \left(\Sigma^{-1} \frac{\partial{\Sigma}}{\partial \theta_i} \Sigma^{-1} \frac{\partial \Sigma}{\partial \theta_j} \right)
\end{align}

to show that the \gls{sfim} for a multiple targets' positions with multiple radars is

\begin{align}
    J(\chi^{T_m}_{xyz};\chi^{R_n}_{xyz}) &= (\chi^{T_m}_{xyz} - \chi^{R_n}_{xyz})(\chi^{T_m}_{xyz} - \chi^{R_n}_{xyz})^T \times \nonumber \\
    &\left( \frac{4}{K \lVert\chi^{R}_{xyz} - \chi^{T}_{xyz} \rVert^6} + \frac{8}{\lVert \chi^{R}_{xyz} - \chi^{T}_{xyz} \rVert^4} \right) \label{eqn:fim_single_radar_single_target} \\
    J(\chi^{T_m}_{xyz};\chi^{R_{1:N}}_{xyz}) &= \sum_{n=1}^N J(\chi^{T_m}_{xyz} ; \chi^{R_n}_{xyz})     \label{eqn:fim_multi_radar_single_target} 
\end{align}

\begin{align}
        &J(\chi^{T_{1:m}}_{xyz};\chi^{R_{1:n}}_{xyz}) = \nonumber \\
        &\begin{bmatrix}
        J(\chi^{T_{1}}_{xyz};\chi^{R_{1:N}}_{xyz}) & 0 & \ldots & 0 \\
        0 & J(\chi^{T_{2}}_{xyz};\chi^{R_{1:N}}_{xyz}) & \ldots & 0 \\
        \vdots & \vdots & \ddots & \vdots \\
        0 & 0 & \ldots & J(\chi^{T_{M}}_{xyz};\chi^{R_{1:N}}_{xyz})
    \end{bmatrix} \label{eqn:fim_multi_radar_multi_target}
\end{align}

When there is prior knowledge about the dynamics of the target state (\cref{eqn:dynamics_single_target}), then this information may be incorporated at the \gls{pfim}:
\begin{align}
    J = J_D + J_P \\
    J_P = E[\Delta_{\chi^T}^{\chi^T} \log f(\chi^T)]
\end{align}

Here, $J_D$ represents the information about the unknown target state obtained from the data, while $J_P$ reflects the information about the unknown target state based on prior assumptions. However, considering that the targets' state includes velocity, we update \cref{eqn:fim_multi_radar_multi_target} for the \gls{pcrlb} as:

\begin{align}
&J(\chi^{T_n};\chi^{R_{1:N}}_{xyz}) =  \begin{bmatrix}
    J(\chi^{T_n}_{xyz};\chi^{R_{1:N}}_{xyz}) & 0 \\
    0 & 0
\end{bmatrix} \\
&J(\chi^{T_{1:m}};\chi^{R_{1:n}}_{xyz}) = \nonumber \\
&\begin{bmatrix}
J(\chi^{T_1};\chi^{R_{1:N}}_{xyz}) & 0 & \ldots & 0 \\
0 & J(\chi^{T_2};\chi^{R_{1:N}}_{xyz}) & \ldots & 0 \\
\vdots & \vdots & \ddots & \vdots \\
0 & 0 & \ldots & J(\chi^{T_M};\chi^{R_{1:N}}_{xyz})
\end{bmatrix} \label{eqn:fim_multi_radar_multi_target_velocity}
\end{align}


Furthermore, an efficient recursive computation of the \gls{pfim} at time step $k+1$ from time step $k$ is \cite{tichavsky1998posterior}
\begin{align}
    &J_{k+1} (\chi^{T_{1:M}}_{k+1}) = D_k^{22} - D_k^{21} (J_k + D_k^{11})^{-1} D_k^{12} \label{eqn:pfim_recursion}
\end{align}
where
\begin{align}
    &D_k^{11} = E[-\Delta_{\chi^{T_{1:M}}_k}^{\chi^{T_{1:M}}_k} \log p(\chi^{T_{1:M}}_{k+1} | \chi^{T_{1:M}}_k)]  \\
    &D_k^{12} = E[-\Delta_{\chi^{T_{1:M}}_k}^{\chi^{T_{1:M}}_{k+1}} \log p(\chi_{k+1} | \chi_k)] = [D_k^{21}]^T \\
    &D_k^{22} = E\left[-\Delta_{\chi^{T_{1:M}}_{k+1}}^{\chi^{T_{1:M}}_{k+1}} \log p(\chi^{T_{1:M}}_{k+1} | \chi^{T_{1:M}}_{k}) \right] + \nonumber \\
    & \qquad E\left[-\Delta_{\chi^{T_{1:M}}_{k+1}}^{\chi^{T_{1:M}}_{k+1}} \log p(z_{k+1} | \chi^{T_{1:M}}_{k+1}) \right] 
\end{align}
which is straightforwardly calculated as 
\begin{align}
    &D_k^{11} =A^T Q^{-1} A  \label{eqn:d11}\\
    &D_k^{12} = - A^T Q^{-1} \label{eqn:d12} \\
    &D_k^{22} =  Q^{-1} + E_{f(\chi^{T_{1:M}}_{1:k+1})} \left[-J_{D_k}(\chi^{T_{1:M}}_{k+1})) \right] \label{eqn:d22}
\end{align}

where due to the Markov assumption on the transition model in the state space equation (\cref{eqn:transition_model}), the joint density $f(\chi^{T_{1:M}}_{1:k})$ is simplified as
\begin{align}
    f(\chi^{T_{1:M}}_{1:k}) = f(\chi^{T_{1:M}}_{0}) \prod_{t=1}^{k+1} f(\chi^{T_{1:M}}_{t} | \chi^{T_{1:M}}_{t-1})
\end{align}


After substituting equations \cref{eqn:d11,eqn:d12,eqn:d22}, \cref{eqn:pfim_recursion} is rewritten as follows for numerical stability, avoiding the inversion of $Q$ \cite{simplifed_pfim_recursion}:

\begin{align}
    J_{k+1} (\chi^{T_{1:M}}_{k+1}) = (Q + A^T J_k^{-1} A)^{-1} + E_{f(\chi^{T_{1:M}}_{1:k+1})} \left[-J_{D_k}(\chi^{T_{1:M}}_{k+1})) \right] \label{eqn:pfim_simplified}
\end{align}


To compute the expectation over the target state for future time steps in either \cref{eqn:pfim_simplified} or \cref{eqn:fim_multi_radar_multi_target}, we use the Cubature Kalman Filter (\gls{ckf}). 

\textcolor{red}{need to rewwrite \cref{eqn:pfim_simplified,eqn:fim_multi_radar_multi_target} based on CKF}
\glspl{ckf} are efficient nonlinear Bayesian filtering algorithms that incorporate the third-order spherical cubature integration rule into the prediction and correction steps of an additive noise Gaussian Kalman filter \cite{sarkka2023bayesian}. We propagate the sigma points of the \gls{ckf} multiple time steps into the future to compute expectations, using a number of sigma points equal to twice the dimension of the state variable.


With the current equations, we can formulate a discrete-time finite-horizon \gls{mpc} objective  utilizing dynamic, control, and mission-aware constraints.


\section{Model Predictive Controller Objective}

\gls{mpc} is an optimal control technique that determines the control actions minimizing a cost function for a constrained dynamical system over a finite, receding horizon \cite{morari1999model,khaled2018practical}. A  state-dependent cost function for given set of radar and target trajectories subject to dynamic constraints is defined as

\begin{equation}
\begin{aligned}
    S_{traj}(\chi^{R_{1:N}}_{1:K} ; \chi^{T_{1:M}}_{1:K}) = \sum_{k=1}^{K} \Phi(\chi^{R_{1:N}}_k;\chi^{T_{1:M}}_K) 
\end{aligned}
\label{eqn:mpc_obj}
\end{equation}

where $\chi_k^{R_{1:N}}$ and $\chi_k^{T_{1:M}}$ obey dynamic constraints in \cref{eqn:dynamics_single_target,eqn:radar_kinematics_constrained}. 

The $\Phi(\cdot)$ is the instantaneous cost, and we define the terminal cost as always 0. In this paper, we define the instantaneous cost from radars' trajectories as $\Phi(\cdot)= -\log \det J(\cdot)$ (or $\Phi(\cdot)= -\log \det J_D(\cdot)$) with the \glspl{fim} defined in \cref{sec:fim_definition}. 

In mission scenarios, ensuring a safe distance between radars and targets is crucial to prevent the adversary from destroying the radars. Similarly, in dynamic radar environments where radars are on moving platforms, maintaining a safe distance between radars is essential to prevent collisions amongst radars or with the environment. Therefore, we include additional constraints, such as the distances among the radars  and the between the radars and the targets, into \cref{eqn:mpc_obj}:

\begin{equation}
\begin{aligned}
    &S_{traj}(\chi^{R_{1:N}}_{1:K} ; \chi^{T_{1:M}}_{1:K}) = \sum_{k=1}^{K} \Phi(\chi^{R_{1:N}}_k;\chi^{T_{1:M}}_{1:K}) \\
    &\text{such that} \\
    &\chi^{R_{n}}_{k+1} =G_k(\chi^{R_{n}}_k) \chi^{R_{n}}_k + B_k u_k \quad \forall n \\
    & \underbar{$u$}_a \leq u_{a_k} \leq \bar{u}_a \;  \quad \forall k \\
    & \underbar{$u$}_{\dot{\omega}} \leq u_{\dot{\omega}_k} \leq \bar{u}_{\dot{\omega}} \;  \quad\forall k  \\
    & \underbar{$v$} \leq v_k \leq \bar{v} \; \quad \forall k \\
    & \underbar{ $\omega$ } \leq \omega_k \leq \bar{ \omega } \; \quad \forall k \\
    & S_{R2T}(\cdot) = \lVert \chi_k^{T_n} - \chi_k^{R_m}  \rVert - R_{R2T} \geq 0 \;  \quad \forall m \; \forall n\\
    & S_{R2R}(\cdot) = \lVert \chi_k^{R_i} - \chi_k^{R_j} \rVert -  R_{R2R} \geq 0 \quad i \in M \; , \;  j \in M / i 
\end{aligned}
\label{eqn:mpc_obj_constrained}
\end{equation}

We may reduce the number of hard constraints in \cref{eqn:mpc_obj_constrained} by converting some hard constraints to soft constraints, absorbing the radar dynamic model constraints into the kinematic model \cite{asmar2023model}, and performing direct shooting method \cite{directshooting} such that the objective simplifies to an unconstrained discontinuous non-differentiable objective formulation

\begin{equation}
\begin{aligned}
    &S(u_{1:K} ; \chi^{T_{1:M}}_{1:K}) = S_{traj}(u_{1:K} ; \chi^{T_{1:M}}_{1:K}) + \alpha_1 S_{R2R}(u_{1:K}) \\
    & \quad \quad \quad  \quad \quad \quad \quad + \alpha_2 S_{R2T}(u_{1:K} ; \chi^{T_{1:M}}_{1:K}) \\
    &\text{where }\\
    & S_{R2T}(u_{1:K}) =  \sum_{m=1}^M \sum_{n=1}^N \mathbf{1} \left( \lVert \chi_k^{T_n} + \chi_k^{R_m}(u_{1:k})  \rVert \leq R_{R2T} \right) \\
    & S_{R2R}(u_{1:K}) =  \sum_{i=1}^M \sum_{i=1,i\neq j}^M \mathbf{1} \left( \lVert \chi_k^{R_i}(u_{1:k}) - \chi_k^{R_j}(u_{1:k})  \rVert \leq R_{R2R} \right) \\
\end{aligned}
\label{eqn:mpc_obj_unconstrained}
\end{equation}

and $\alpha_1,\alpha_2$ are hyperparameters that determine how much to penalize the radars for violating the soft constraints $S_{R2R},S_{R2T}$ respectively.

\begin{figure*}[h!]
    \centering
    \includegraphics[width=18cm]{images/example.jpg}
    \caption{To be filled}
    \label{fig:mppi_example}
\end{figure*}

Due to the uncertainty in the target states, we compute the expectation of \cref{eqn:mpc_obj_unconstrained} with respect to the \gls{ckf} on the target states. This involves averaging the objective function over the evaluations at the sigma points of the \gls{ckf} and the forward propagated sigma points of the \gls{ckf}.

\begin{equation}
\begin{aligned}
    &S(u_{1:K} ; \chi^{T_{1:M}}_{1:K}) = E_{\tilde{f}(\chi_{1:K}^{T_{1:M}})}S_{traj}(u_{1:K} ; \chi^{T_{1:M}}_{1:K}) - \alpha_1 S_{R2R}(u_{1:K}) \\
    & \quad \quad \quad  \quad- \alpha_2 E_{\tilde{f}(\chi_{1:K}^{T_{1:M}})} \left[ S_{R2T}(u_{1:K} ; \chi^{T_{1:M}}_{1:K}) \right] \\
    &\tilde{f}(\chi_{1:K}^{T_{1:M}}) = f_{ckf}(\chi^{T_{1:M}}_{k}|\mathbf{z}_{1:k-1}) \prod_{t=k+1}^{k+K+1} f(\chi^{T_{1:M}}_{t} | \chi^{T_{1:M}}_{t-1})
\end{aligned}
\label{eqn:expected_mpc_obj_unconstrainted}
\end{equation}

We use \gls{mppi} to estimate the optimal control inputs to the radars due to the advantage of directly accounting for noise characteristics and dynamics of the vehicles during optimization \cite{williams2018information}, the cost function may be defined with fewer restrictions such as smoothness,  high parallelization, and control input adaptability \cite{mppi_advantages}

\subsection{Model Predictive Path Integral}
\gls{mppi} is a sampling-based model predictive control algorithm designed for optimizing non-linear stochastic systems subject to complex cost functions in real time \cite{7487277}. The assumption of \gls{mppi} is that we do not have direct control over the control input variable $u$, but that the control input is random and distributed as Gaussian random vector $v \sim N(u,\Sigma)$. Due to the stochasticity on the control input, rather than solving for a deterministic optimal control input we solve for an optimal control density $Q^*$ \cite{theodorou2010generalized}. 
The optimal control density might not possess an analytical form; therefore, we utilize variational inference to approximate $Q^*$ by minimizing the Kullback-Leibler Divergence of $Q^*$ with a Gaussian density parameterized by $u,\Sigma$ \cite{williams2018information}: 
\begin{align}
    u_{1:K}^* = \arg \min_{u_{1:K},\Sigma} D_{KL} (Q^*,Q_{u_{1:K},\Sigma}) \label{eqn:kl_mppi}
\end{align}

where $Q^* = \frac{1}{\eta} \exp\left(-\frac{1}{b}S(v_{1:K}) \right) P(v_{1:K}) $ and $P(\cdot)$ is the probability density of an control input sequence in an uncontrolled system ($u_{1:K} = 0)$ \cite{williams2018information}. $b$ is the temperature of the distribution, and $\eta$ is the evidence.

\cref{eqn:kl_mppi} is solved using \gls{ais} as follows: 
\begin{enumerate}
    \item sample control trajectories $v_{1:k}^{(i)}$ from distribution $Q$ with mean $u_{1:K}$ and covariance $\Sigma$
    \item evaluate the objective function for each control trajectory sample $S(v_{1:K}^{(i)})$
    \item compute the importance sampling corrective weights for each sample as proportional to $\tilde{w}^{(i)} \propto S(v^{(i)})$
    \item adapt the mean and covariance of the density $Q$ 
    \item repeat steps 1-4
\end{enumerate}
\cite{asmar2023model,williams2018information}.


However, due to high dimensionality of the targets state, 


==> methodology/methodology_draft2.tex <==
\section{Radar Signal Model}
\label{sec:radar_signal_model}
Following the approach in \cite{godrich2010target}, we assume there are $N$ radars transmitting orthogonal narrowband signals to track $M$ targets (employing time division multiplexing to track multiple targets). In this setup, the received signal at radar $n$ for target $m$ is given by:
%
\begin{align}
    r^{nm}(t) &= \sum_{b=1}^N \zeta^{nm} e^{-j2\pi f_c \tau^{nm}} s^b(t-\tau^{nm}) + \epsilon_{a}^n(t), \label{eqn:return_signal} 
\end{align}
where the time delay is:
\begin{align}
    \tau^{nm} &= \frac{\lVert \chi^{R_n}_{xyz} - \chi^{T_m}_{xyz} \rVert  +  \lVert \chi^{R_b}_{xyz} - \chi^{T_m}_{xyz} \rVert} {c},
\end{align}
%
and the set of lowpass equivalent signals $s(t)$ are orthonormal such that
\begin{align}
    \int_T s^i(t) s^j(t) dt = \begin{cases}
        0 & i\neq j \\
        1 & i=j
    \end{cases} \label{eqn:orthogonality}
\end{align} 
The return signal noise $\epsilon_{a}(t)$ is circularly symmetric, zero-mean, complex Gaussian noise with autocorrelation function $\sigma_a^2 \delta (\tau)$. We define $\zeta$ as the complex amplitude of the return signal, where $|\zeta|^2$ is the radar power return specified by the radar equation \cite{barton2013radar}:
\begin{align}
    |\zeta|^2 = P_r = \frac{P_t \Lambda_t \Lambda_r \lambda^2 \Xi}{(4\pi)^3 \lVert \chi^{R}_{xyz} - \chi^{T}_{xyz} \rVert ^4 L}
\end{align}
The radar parameters specifying the received power $P_r$ $[W]$ at the radar include $P_t$ as the transmit power $[W]$, $\Lambda_t$ and $\Lambda_r$ as the transmit and receive gains, $L$ as the general loss factor, $\Xi$ as the radar cross section $[m^2]$, and $\lambda$ as the carrier frequency wavelength $[m]$.

By maximizing a second-order Taylor series expansion centered at $\tau^{nm}$ of the match filter between the expected return signal and the received return signal with respect to the time delay $\tau^{nm}$, it has been shown that the time delay between radar $n$ and target $m$ follows a Gaussian \gls{pdf} with variance parameterized by the radar-target geometry.
\begin{align}
    z^{nm} &= \tau^{nm} + \epsilon_z^{nm} \label{eqn:tod_measurement}\\
    \epsilon_z^{nm} &\sim \mathcal{N}\left(0,\frac{\sigma_a^2}{8\pi^2 f_c^2 |\zeta^{nm}|^2} \right) 
\end{align}

The \gls{pdf} over radar-target paired range measurements is obtained by multiplying \cref{eqn:tod_measurement} by the speed of light $c$ on both the left-hand side (LHS) and the right-hand side (RHS):

\begin{align}
z^{nm} \sim  \mathcal{N}\left(2 \lVert \chi^{R_n}_{xyz} - \chi^{T_m}_{xyz} \rVert \; , \; \frac{c^2 \sigma_a^2}{8\pi^2 f_c^2 |\zeta^{nm}|^2} \right) \label{eqn:range_measurement}
\end{align}

We denote all the radar parameters, signal parameters, and noise parameters as a constant $K=\frac{c^2 \sigma_a^2 (4\pi)^3 L}{P_t \Lambda_t \Lambda_r \lambda ^2 \Xi 8\pi^2 f_c^2} $. For brevity, we define shorthand notation  as 
$h^{nm} = 2 \lVert \chi^{R_n}_{xyz} - \chi^{T_m}_{xyz} \rVert $ and $\sigma_z^{nm} = \frac{c^2 \sigma_a^2}{8\pi^2 f_c^2 |\zeta^{nm}|^2}$.

Existing research has explored optimal radar placement when the covariance matrix of the range measurement depends on the radar-target geometry \cite{moreno2011optimal,yan2017exact,he2015generalized}, primarily focusing on stationary targets and radars.

Given that the range measurement model relies on the positions of both the radars and targets, the next section describes the target and radar kinematic models. This will facilitate the definition of the targets' conditional transition probability in the targets' state space model.


\section{Process Model}
\label{sec:process_modeling}
We describe the kinematic model of a target to finalize the probabilistic state space model for the concatenated state of all the targets, encompassing both a conditional transition probability and the conditional measurement probability described in \ref{sec:radar_signal_model}.

\subsection{Target Kinematics: Constant Velocity Model}
Following \cite{baisa2020derivation}, we define the assumed target kinematic model for a single target undergoing constant velocity motion with acceleration noise, which specifies the conditional transition probability of a single target as:
\begin{align}
\chi^T_{k+1} &= A\chi_k^T + \epsilon_w \label{eqn:dynamics_single_target} 
\end{align}
where 
\begin{align}
    A_{\text{single}} &= \begin{bmatrix}
        1 & 0 & 0 & \Delta t & 0 & 0 \\ 
        0 & 1 & 0 & 0 & \Delta t & 0 \\ 
        0 & 0 & 1 & 0 & 0 & \Delta t \\ 
        0 & 0 & 0 & 1 & 0 & 0 \\
        0 & 0 & 0 & 0 & 1 & 0 \\
        0 & 0 & 0 & 0 & 0 & 1 \\
    \end{bmatrix} \\ 
\end{align}
and $\epsilon_w$ is the acceleration noise which follows a Gaussian \gls{pdf} with covariance
\begin{align}
         W_{\text{single}} &= \begin{bmatrix}
        \frac{\Delta t^4}{4} & 0 & 0 & \frac{\Delta t^3}{2} & 0 & 0 \\ 
        0 & \frac{\Delta t^4}{4} & 0 & 0 & \frac{\Delta t^3}{2} & 0 \\ 
        0 & 0 & \frac{\Delta t^4}{4} & 0 & 0 & \frac{\Delta t^3}{2}\\ 
        \frac{\Delta t^3}{2} & 0 & 0 & \Delta t^2 & 0 & 0 \\
        0 & \frac{\Delta t^3}{2} & 0 & 0 & \Delta t^2 & 0 \\
        0 & 0 & \frac{\Delta t^3}{2} & 0 & 0 & \Delta t^2\\
    \end{bmatrix} \cdot \sigma_W^2
\end{align}
Thus, the conditional transition \gls{pdf} for the targets' state-space equations is defined as
\begin{align}
    A &= I_{M} \otimes A_{\text{single}} \\
    W &= I_{M} \otimes W_{\text{single}} \\
     \chi^{T_{1:M}}_{k+1} &= A \chi^{T_{1:M}}_k + \epsilon_{W} \label{eqn:transition_model} 
\end{align}
with $M \times M$-dimensional identity matrix $I_{M}$.

Similarly, the measurements of all radar-target pairs may be concatenated for the conditional measurement \gls{pdf} of the targets' state-space equations (based on \cref{eqn:range_measurement}):

\begin{align}
\mathbf{z}^{T_{1:M}} &= \begin{bmatrix}
h^{11} & \ldots & h^{1M} \\
h^{21} & \ldots & h^{2M} \\
\vdots & \ddots & \vdots \\
h^{N1} & \ldots & h^{NM} \\
\end{bmatrix} +  \begin{bmatrix}
\sigma_z^{11} & \ldots & \sigma_z^{1M} \\
\sigma_z^{21}  & \ldots & \sigma_z^{2M}  \\
\vdots & \ddots & \vdots \\
\sigma_z^{NM} & \ldots & \sigma_z^{nM}  \\
\end{bmatrix} \odot \epsilon_\mathbf{z} \label{eqn:measurement_prob} \\
&= \mathbf{H(\chi^{T_{1:M}}_{xyz}}) + \Omega \odot \sigma_\mathbf{z}
\end{align}

where $\sigma_z^{nm}$ is the standard deviation of the range measurement for radar $n$ and target $m$, as defined by the variance in \cref{eqn:range_measurement}, while $\sigma_z$ is standard normal Gaussian \gls{pdf}.

Therefore the final state-space equations for the targets is shown in \cref{eqn:state_space_meas,eqn:state_space_tran}:

\begin{align}
     \chi^{T_{1:M}}_{k+1} &= A\chi^{T_{1:M}}_k + \epsilon_{W} \label{eqn:state_space_tran} \\
    \mathbf{z}^{T_{1:M}}_{k+1} &= \mathbf{H}\left((\chi^{T_{1:M}}_{xyz})_{k+1}\right) + \Omega \odot \sigma_\mathbf{z} \label{eqn:state_space_meas} 
\end{align}

Given our focus on dynamic targets and dynamic radars, it's essential to outline a basic kinematic model where the radar position is determined by control inputs and adheres to specific control and dynamic constraints. Thus, we next define the second-order unicycle kinematic model for the radars.

\subsection{Radar Kinematics: Second-Order Unicycle Model}

Each radar follows the second-order unicycle model. We use the Euler discretization of the unicycle continuous dynamic model with heading acceleration and angular acceleration control inputs $u = [u_{a},u_{\dot{\omega}}]^T$ to define the discrete time kinematic model:

% x_{k+1} &= x_{k} + \dot{x}_k \cos{\theta_k} \Delta t + \frac{1}{2} (u_{a})_k \cos{\theta_k} \Delta t^2  \\
% y_{k+1} &= y_{k} + \dot{y}_k \sin{\theta_k} \Delta t + \frac{1}{2} 
% (u_{a})_k \sin{\theta_k} \Delta t^2 \\
% z_{k+1} &= z_{k} \\
% \theta_{k+1} &= \theta_{k} + \omega_k \Delta t + \frac{1}{2} u_{\dot{\omega}_k} \Delta t^2 \\
% v_{k+1} &= v_k + (u_{a})_k \Delta t \\
% \omega_{k+1} &= \omega_{k} + (u_{\dot{\omega}})_k \Delta t \\

\begin{equation}
\begin{aligned}
    \begin{bmatrix}
        x_{k+1} \\
        y_{k+1} \\
        z_{k+1} \\
        \theta_{k+1} \\
        v_{k+1} \\ 
        \omega_{k+1}
    \end{bmatrix} &=
    \begin{bmatrix}
        1 &  0 & 0 & 0 & \cos \theta_k \Delta t & 0 \\
        0 & 1 & 0 & 0 & \sin \theta_k \Delta t & 0\\
        0 & 0 & 1 & 0 & 0 & 0 \\
        0 & 0 & 0 & 1 & 0 & \Delta t  \\
         0 & 0 & 0 & 0 & 1 & 0  \\
        0 & 0 & 0 & 0 & 0 & 1
    \end{bmatrix} 
        \begin{bmatrix}
        x_{k} \\
        y_{k} \\
        z_{k} \\
        \theta_{k} \\
        v_{k} \\
        \omega_{k}
    \end{bmatrix} +  \\ 
    & \begin{bmatrix}
     \frac{1}{2} \cos \theta_k \Delta t^2 & 0 \\
     \frac{1}{2} \sin \theta_k \Delta t^2 & 0 \\
    0  & 0  \\
    0  & \frac{1}{2} \Delta t^2 \\
    \Delta t & 0\\
        0 & \Delta t 
    \end{bmatrix} u_k \\
    \chi^{R}_{k+1} &= \chi^{R}_k + G_k(\chi^{R}_k,u_k)
\end{aligned}
        \label{eqn:radar_kinematics}
\end{equation}
with control, velocity, and angular velocity limits,
\begin{equation}
\begin{aligned}
\begin{split}
\underbar{$u$}_a \leq u_{a_k} &\leq \bar{u}_a \; \forall k \\
\underbar{$u$}_{\dot{\omega}} \leq u_{\dot{\omega}_k} &\leq \bar{u}_{\dot{\omega}} \; \forall k  \\
\end{split} \quad
\begin{split}
\underbar{$v$} \leq v_k &\leq \bar{v} \; \forall k \\
\underbar{$\omega$} \leq \omega_k &\leq \bar{ \omega } \; \forall k.
\end{split}
\end{aligned}
\label{eqn:radar_kinematics_constrained}
\end{equation}


With the radar's position defined relative to control inputs, the following section outlines the derivation of the \gls{sfim} for the targets' positions, which is parameterized by the radar's control inputs. This is based on the radar-target measurement model outlined in Equations \cref{eqn:range_measurement,eqn:measurement_prob}, and the radar's position parameterized by Equations \cref{eqn:radar_kinematics,eqn:radar_kinematics_constrained}.

\section{Fisher Information Matrix}
\label{sec:fim_definition}

The \gls{sfim} measures the amount of information that an observable random variable $z$ (range measurements) carries about an unknown parameter $\theta$ (targets' states) \cite{tichavsky1998posterior,kay1993fundamentals}:

\begin{align}
    J_D(\theta) = E\left[\left( \nabla_{\theta} \log f\left(z|\theta \right) \right) \left( \nabla_{\theta} \log f\left(z|\theta \right) \right)^T\right]
\end{align}

Under the assumption of independence, the likelihood of the range measurements in \cref{eqn:measurement_prob} is represented as:
\begin{align}
    f\left(\mathbf{z}^{T_{1:M}}|\chi^{T_{1:M}}_{xyz} ; \chi^{R_{1:N}}_{xyz} \right) &= \prod_{n=1}^{N} \prod_{m=1}^{M} f(z^{nm} | \chi^{T_m}_{xyz} ; \chi^{R_n}_{xyz})
\end{align}

and the log likelihood is 
\begin{align}
    \log  f(\mathbf{z}^{T_{1:M}}|\chi^{T_{1:M}}_{xyz} ; \chi^{R_{1:N}}_{xyz}) &= \sum_{n=1}^{N} \sum_{m=1}^{M} \log f(z^{nm} | \chi^{T_m}_{xyz} ; \chi^{R_n}_{xyz}) 
\end{align}

Given that the measurement follows a Gaussian \gls{pdf}, where the mean and covariance are parameterized by the targets' positions, and that information of measurements is additive under the assumption of independence, we can utilize the derivation of general Gaussian \gls{fim} \cite{kay1993statistical}: 

\begin{align}
    \mathbf{z}^{T_{1:M}} &\sim \mathcal{N}(\mu(\theta),\Sigma(\theta)) \\
    (J_{D})_{\theta_i,\theta_j} &= \frac{\partial \mu^T}{\partial \theta_i} \Sigma^{-1} \frac{\partial \mu}{\partial \theta_j} + \frac{1}{2} Tr \left(\Sigma^{-1} \frac{\partial{\Sigma}}{\partial \theta_i} \Sigma^{-1} \frac{\partial \Sigma}{\partial \theta_j} \right)
\end{align}

to show that the \gls{sfim} for a multiple targets' positions with multiple radars is

\begin{align}
    J(\chi^{T_m}_{xyz};\chi^{R_n}_{xyz}) &= (\chi^{T_m}_{xyz} - \chi^{R_n}_{xyz})(\chi^{T_m}_{xyz} - \chi^{R_n}_{xyz})^T \times \nonumber \\
    &\left( \frac{4}{K \lVert\chi^{R}_{xyz} - \chi^{T}_{xyz} \rVert^6} + \frac{8}{\lVert \chi^{R}_{xyz} - \chi^{T}_{xyz} \rVert^4} \right) \label{eqn:fim_single_radar_single_target} \\
    J(\chi^{T_m}_{xyz};\chi^{R_{1:N}}_{xyz}) &= \sum_{n=1}^N J(\chi^{T_m}_{xyz} ; \chi^{R_n}_{xyz})     \label{eqn:fim_multi_radar_single_target} 
\end{align}

\begin{align}
        &J(\chi^{T_{1:m}}_{xyz};\chi^{R_{1:n}}_{xyz}) = \nonumber \\
        &\begin{bmatrix}
        J(\chi^{T_{1}}_{xyz};\chi^{R_{1:N}}_{xyz}) & 0 & \ldots & 0 \\
        0 & J(\chi^{T_{2}}_{xyz};\chi^{R_{1:N}}_{xyz}) & \ldots & 0 \\
        \vdots & \vdots & \ddots & \vdots \\
        0 & 0 & \ldots & J(\chi^{T_{M}}_{xyz};\chi^{R_{1:N}}_{xyz})
    \end{bmatrix} \label{eqn:fim_multi_radar_multi_target}
\end{align}

where equation \cref{eqn:fim_single_radar_single_target} is the \gls{sfim} of a single target position parameterized by a single radar and \cref{eqn:fim_multi_radar_single_target} is the \gls{sfim} of a single target positions parameterized by multiple radars.

When there is prior knowledge about the dynamics of the target state (\cref{eqn:dynamics_single_target}), then this information may be incorporated into the \gls{sfim} to form the \gls{pfim}:
\begin{align}
    J = J_D + J_P \\
    J_P = E[\Delta_{\chi^T}^{\chi^T} \log f(\chi^T)] \label{eqn:pfim_single}
\end{align}

Here, $J_D$ represents the information about the unknown target state obtained from the data, while $J_P$ reflects the information about the unknown target state based on prior assumptions. However, considering that the targets' state includes velocity, we update \cref{eqn:fim_multi_radar_single_target,eqn:fim_multi_radar_multi_target} for the \gls{pfim} as:

\begin{align}
&J(\chi^{T_n};\chi^{R_{1:N}}_{xyz}) =  \begin{bmatrix}
    J(\chi^{T_n}_{xyz};\chi^{R_{1:N}}_{xyz}) & 0 \\
    0 & 0
\end{bmatrix} \\
&J(\chi^{T_{1:m}};\chi^{R_{1:n}}_{xyz}) = \nonumber \\
&\begin{bmatrix}
J(\chi^{T_1};\chi^{R_{1:N}}_{xyz}) & 0 & \ldots & 0 \\
0 & J(\chi^{T_2};\chi^{R_{1:N}}_{xyz}) & \ldots & 0 \\
\vdots & \vdots & \ddots & \vdots \\
0 & 0 & \ldots & J(\chi^{T_M};\chi^{R_{1:N}}_{xyz})
\end{bmatrix} \label{eqn:fim_multi_radar_multi_target_velocity}
\end{align}

For discrete time filtering systems, such as \cref{eqn:state_space_meas,eqn:state_space_tran}, the
\cref{eqn:pfim_single} is recursively computed at time $k+1$ from time step $k$ using the famous recursion in \cite{tichavsky1998posterior}. The recursion equations are written as 
\begin{align}
    &J_{k+1} (\chi^{T_{1:M}}_{k+1}) = D_k^{22} - D_k^{21} (J_k + D_k^{11})^{-1} D_k^{12} \label{eqn:pfim_recursion}
\end{align}
where
\begin{align}
    &D_k^{11} = E[-\Delta_{\chi^{T_{1:M}}_k}^{\chi^{T_{1:M}}_k} \log p(\chi^{T_{1:M}}_{k+1} | \chi^{T_{1:M}}_k)]  \\
    &D_k^{12} = E[-\Delta_{\chi^{T_{1:M}}_k}^{\chi^{T_{1:M}}_{k+1}} \log p(\chi_{k+1} | \chi_k)] = [D_k^{21}]^T \\
    &D_k^{22} = E\left[-\Delta_{\chi^{T_{1:M}}_{k+1}}^{\chi^{T_{1:M}}_{k+1}} \log p(\chi^{T_{1:M}}_{k+1} | \chi^{T_{1:M}}_{k}) \right] + \nonumber \\
    & \qquad E\left[-\Delta_{\chi^{T_{1:M}}_{k+1}}^{\chi^{T_{1:M}}_{k+1}} \log p(z_{k+1} | \chi^{T_{1:M}}_{k+1}) \right] 
\end{align}

Each $D$ term in equation \cref{eqn:pfim_recursion} is straightforwardly calculated (with some algebraic manipulation and \gls{pdf} regularity assumptions) as 

\begin{align}
    &D_k^{11} =A^T W^{-1} A  \label{eqn:d11}\\
    &D_k^{12} = - A^T W^{-1} \label{eqn:d12} \\
    &D_k^{22} =  W^{-1} + E_{f(\chi^{T_{1:M}}_{1:k+1})} \left[-J_{D_k}(\chi^{T_{1:M}}_{k+1})) \right] \label{eqn:d22}
\end{align}

where due to the Markov assumption on the transition model in the targets' state space equation (\cref{eqn:transition_model}), the joint \gls{pdf} $f(\chi^{T_{1:M}}_{1:k})$ is simplified as
\begin{align}
    f(\chi^{T_{1:M}}_{1:k}) = f(\chi^{T_{1:M}}_{0}) \prod_{t=1}^{k+1} f(\chi^{T_{1:M}}_{t} | \chi^{T_{1:M}}_{t-1}) \label{eqn:markov_simplified}
\end{align}


After substituting equations \cref{eqn:d11,eqn:d12,eqn:d22} into \cref{eqn:pfim_recursion}, and leveraging the Woodbury matrix identity \cite{bishop2006pattern}, we arrive at  \cite{simplifed_pfim_recursion}:

\begin{align}
    J_{k+1} (\chi^{T_{1:M}}_{k+1}) = (W + A^T J_k^{-1} A)^{-1} + E_{f(\chi^{T_{1:M}}_{1:k+1})} \left[-J_{D_k}(\chi^{T_{1:M}}_{k+1})) \right] \label{eqn:pfim_simplified}
\end{align}

\cref{eqn:pfim_simplified} is preferred over \cref{eqn:pfim_recursion} for numerical stability. This preference arises because it avoids the inversion of the $W$ matrix, which can be close to singular in cases where the conditional transition PDF is described by constant velocity models.


To compute the expectation over the target state for \cref{eqn:d22}, as well as objective terms involving \cref{eqn:fim_multi_radar_multi_target} or any other objective term in the \gls{mpc} objective that involves the targets' states, we employ the \gls{ckf} to describe \cref{eqn:markov_simplified}.

\glspl{ckf} efficiently leverages third-order spherical cubature integration into both the prediction and correction steps of an additive noise Gaussian Kalman filter \cite{sarkka2023bayesian}. To compute the expectations described in the previous paragraph, we propagate the sigma points of the \gls{ckf} multiple time steps into the future, employing a number of sigma points equal to twice the dimension of the state variable. Compared to a \gls{pf}, the \gls{ckf} offers lower computational complexity, as the number of evaluation points scales linearly with the state size, whereas the number of particles in a \gls{pf} may grow substantially larger.


With our current formulations in \cref{sec:radar_signal_model,sec:process_modeling,sec:fim_definition}, we next formulate a discrete-time finite-horizon \gls{mpc} objective  utilizing dynamic, control, and mission-aware constraints.


\section{Model Predictive Controller Objective}
\label{sec:mpc_objective}
\gls{mpc} is an optimal control technique that determines the control actuation minimizing a cost function for a constrained dynamical system over a finite, receding horizon \cite{morari1999model,khaled2018practical}. A state-dependent cost function $S_\text{traj}$ for given set of radar and target trajectories subject to dynamic constraints beginning at time point $t$ is defined as
\begin{align}
    S_{traj}\left(\chi^{R_{1:N}}_{k:k+K} ; \chi^{T_{1:M}}_{k:k+K}\right) = \sum_{t=k}^{k+K} \gamma^{t-k}\Phi(\chi^{R_{1:N}}_t;\chi^{T_{1:M}}_t)  \label{eqn:mpc_obj}
\end{align}
where $\chi_k^{R_{1:N}}$ and $\chi_k^{T_{1:M}}$ obey dynamic constraints in \cref{eqn:dynamics_single_target,eqn:radar_kinematics_constrained}, $\Phi(\cdot)$ is the instantaneous cost, $\gamma$ the discount factor, and we define the terminal cost as always 0. In this paper, we define the instantaneous cost from radars' trajectories as $\Phi(\cdot)= -\log \det J(\cdot)$ (or $\Phi(\cdot)= -\log \det J_D(\cdot)$) with the \glspl{fim} defined in \cref{sec:fim_definition}. 
In mission scenarios, ensuring a safe distance between radars and targets is crucial to prevent the adversary from destroying the radars. Similarly, ensuring a safe separation distance between mobile radars is crucial to avoid collisions either between radars or with the surrounding environment. Therefore, we include additional constraints, such as the distances amongst the radars  and the between radars and targets, into \cref{eqn:mpc_obj}:
\begin{align}
    &S_{traj}\left(\chi^{R_{1:N}}_{k:k+K} ; \chi^{T_{1:M}}_{k:k+K}\right) = \sum_{t=k}^{k+K} \gamma^{t-k} \Phi(\chi^{R_{1:N}}_t;\chi^{T_{1:M}}_{t}) \notag \\
    &\text{such that} \notag \\
    &\chi^{R_{n}}_{k+1} = \chi^{R_{n}}_k + G_k(\chi^{R}_k,u^{R_n}_k) \quad \forall n \; \forall k \notag \\
    & \underbar{$u$}_a \leq u^{R_n}_{a_k} \leq \bar{u}_a \;  \quad \forall n \; \forall k \notag \\
    & \underbar{$u$}_{\dot{\omega}} \leq u^{R_n}_{\dot{\omega}_k} \leq \bar{u}_{\dot{\omega}} \; \quad \forall n \; \forall k  \notag \\
    & \underbar{$v$} \leq v^{R_n}_k \leq \bar{v} \; \quad 
 \forall n \; \forall k \notag \\
    & \underbar{ $\omega$ } \leq \omega_k^{R_n} \leq \bar{ \omega } \; \quad  \forall n \; \forall k \notag \\
    & S_{R2T}(\cdot) = \lVert \chi_k^{T_n} - \chi_k^{R_m}  \rVert - R_{R2T} \geq 0 \;  \quad \forall m \; \forall n \; \forall k \notag \\
    & S_{R2R}(\cdot) = \lVert \chi_k^{R_i} - \chi_k^{R_j} \rVert -  R_{R2R} \geq 0 \quad i \in M ,  j \in M  / i , \forall k 
\label{eqn:mpc_obj_constrained}
\end{align}
%     \begin{figure*}[b]
%     \rule{\textwidth}{1pt}
%     \begin{equation}
% \begin{aligned}
% R = \begin{bmatrix} 
% c\theta+n_1^2(1-c\theta) & n_1n_2(1-c\theta)-n_3s\theta     
%     &   n_1n_3(1-c\theta)+n_2s\theta    \\
% n_2n_1(1-c\theta)+n_3s\theta 
%     &   c\theta+n_2^2(1-c\theta) 
%     & n_2n_3(1-c\theta)-n_1s\theta      \\
% n_3n_1 (1-c\theta)-n_2s\theta 
%     & n_3n_2(1-c\theta)+n_1s\theta & c\theta+n_3^2(1-c\theta)
%     \end{bmatrix}.
% \end{aligned}
%     \end{equation}
%     \end{figure*}
We can reduce the number of hard constraints in \cref{eqn:mpc_obj_constrained} by converting some of them into soft constraints. Additionally, we can absorb the radar dynamic model constraints into the kinematic model \cite{asmar2023model}, and use the direct shooting method \cite{directshooting}. This simplifies the objective to an unconstrained, discontinuous, non-differentiable formulation:

% \begin{equation}
\begin{align}
\hspace{-3cm}
    &S(u_{k:k+K} ; \chi^{T_{1:M}}_{k:k+K}) = S_{traj}(u_{k:k+K} ; \chi^{T_{1:M}}_{k:k+K}) \notag \\
    & \quad \quad \quad  \quad \quad \quad \quad  + \alpha_1 S_{R2R}(u_{k:k+K}) \notag \\
    & \quad \quad \quad  \quad \quad \quad \quad + \alpha_2 S_{R2T}(u_{k:k+K} ; \chi^{T_{1:M}}_{k:k+K}) \notag \\
    &\text{where } \notag\\
    & S_{R2T}(u_{k:k+K} \!) \! = \notag \\
    &\quad  \quad \; \; \!\! \sum_{t=k}^{k+K} \!\! \gamma^{t-k} \!\! \sum_{m=1}^M \! \sum_{n=1}^N \! \mathbf{1} \! \left( \lVert \chi_t^{T_n} \! + \! \chi_t^{R_m}(u_{t})  \rVert \! \leq \! R_{R2T} \! \right) \notag \\
    & S_{R2R}(u_{k:k+K}) = \notag \\
    & \quad  \quad \; \sum_{t=k}^{k+K} \gamma^{t-k} \!\!\!\!\!\! \sum_{\{i<j: i,j \in M\}} \!\!\!\!\!\! \mathbf{1} \left( \lVert \chi_t^{R_i}(u_{t}) - \chi_t^{R_j}(u_{t})  \rVert \leq R_{R2R} \right) 
\label{eqn:mpc_obj_unconstrained}
\end{align}
% \end{equation}

and $\alpha_1,\alpha_2$ are hyperparameters that determine how much to penalize the radars for violating the soft constraints $S_{R2R},S_{R2T}$ respectively.

Due to the uncertainty in the targets' states, we compute the expectation of \cref{eqn:mpc_obj_unconstrained} with respect to the \gls{ckf} estimator of the target states. This involves averaging the objective function over the evaluations at the \gls{ckf} sigma points and the forward propagated \gls{ckf} sigma points based on the targets' state transition function \cref{eqn:dynamics_single_target}.

\begin{equation}
\begin{aligned}
    &S(u_{1:K} ; \chi^{T_{1:M}}_{1:K}) = E_{\tilde{f} (\chi_{1:K}^{T_{1:M}})}\bigg[S_{traj}(u_{1:K} ; \chi^{T_{1:M}}_{1:K}) \\
    & \quad \quad \quad  \quad \quad \quad - \alpha_1 S_{R2R}(u_{1:K}) \\
    & \quad \quad \quad  \quad \quad \quad - \alpha_2 E_{\tilde{f}(\chi_{1:K}^{T_{1:M}})} \left[ S_{R2T}(u_{1:K} ; \chi^{T_{1:M}}_{1:K}) \right] \bigg] \\
    &\tilde{f}(\chi_{1:K}^{T_{1:M}}) = f_{ckf}(\chi^{T_{1:M}}_{k}|\mathbf{z}_{1:k-1}) \prod_{t=k+1}^{k+K+1} f(\chi^{T_{1:M}}_{t} | \chi^{T_{1:M}}_{t-1})
\end{aligned}
\label{eqn:expected_mpc_obj_unconstrainted}
\end{equation}

This \gls{mpc} problem requires an efficient solver that can handle highly nonlinear, discontinuous, and non-differentiable functions. Therefore, we employ a sampling-based strategy, \gls{mppi} \cite{williams2018information}, as discussed in the following section.

\subsection{Model Predictive Path Integral}
\gls{mppi} is a sampling-based \gls{mpc} algorithm designed for optimizing nonlinear stochastic systems subject to complex cost functions in real time \cite{7487277}. The assumption of \gls{mppi} is that we do not have direct control over the control input variable $u$, but that the control input is random and distributed as Gaussian random vector $v \sim N(u,\Sigma)$. Due to the stochasticity on the control input, rather than solving for a deterministic optimal control input we solve for an optimal control \gls{pdf} $Q^*$ \cite{theodorou2010generalized}. 
The optimal control \gls{pdf} might not possess an analytical form; therefore, we use variational inference to approximate $Q^*$ by minimizing the \gls{kbl} of $Q^*$ with a Gaussian \gls{pdf} parameterized by $u,\Sigma$ \cite{williams2018information}: 
\begin{align}
    u_{k:k+K}^* = \arg \min_{u_{k:k+K},\Sigma} D_{KL} (Q^*,Q_{u_{k:k+K},\Sigma}) \label{eqn:kl_mppi}
\end{align}

The optimal control \gls{pdf} is shaped by the \gls{mpc} objective, and is similar to Boltzmann distributions: 

\begin{align}
    Q^* = \frac{1}{\eta} \exp\left(-\frac{1}{b}S(v_{1:K}) \right) P(v_{1:K})
\end{align}

where $P(\cdot)$ is the \gls{pdf} of an control input sequence in an uncontrolled system ($u_{k:k+K} = 0)$ \cite{williams2018information}, $b$ is the temperature of the distribution, and $\eta$ is the evidence. By differentiating \cref{eqn:kl_mppi} with respect to $u_k$, we write the optimal control at $k$ as \cite{williams2018information}
\begin{align}
    u^*_k = \int q^*(V) v_k dV \label{eqn:optimal_control_mppi}
\end{align}

Since we cannot express $Q^*$ analytically in \cref{eqn:optimal_control_mppi}, we leverage \gls{ais} to approximate the expectation as follows: 
\begin{enumerate}
    \item sample control trajectories $v_{1:k}^{(i)}$ from distribution $Q$ with mean $u_{k:k+K}$ and covariance $\Sigma$
    \item evaluate the objective function for each control trajectory sample $S(v_{k:k+K}^{(i)})$
    \item compute the importance sampling corrective weights for each sample as proportional to $\tilde{w}^{(i)} \propto S(v^{(i)})$
    \item adapt the mean and covariance of the \gls{pdf} $Q$ 
    \item repeat steps 1-4
\end{enumerate}
\cite{asmar2023model,williams2018information}.

Because the targets' control input spans a high dimensionality across a horizon, and the number of samples at step 1 of \gls{mppi} is low, the sample covariance matrix for the control inputs often overfits, leading to smaller or larger variances than the true covariance \cite{theiler2012incredible}. As a consequence, the proposal distribution of \gls{mppi} often yields poor control inputs. To address this issue, we adopt the \gls{lw} for the \gls{ais} (which asymptotically approaches the \gls{oas} shrinkage with infinite number of estimation samples), following the approach outlined in \cite{asmar2023model}.

\begin{figure*}[h!]

\centering
\subfigure[Our method: Each radar moves towards the targets.]{\includegraphics[width=8.5cm]{images/sfim1/MPPI_CKF_16.png}}\hfil
\subfigure[\cite{hung2020range,bishop2010optimality,crasta2018multiple} range model: The upper right radar moves away from targets]{\includegraphics[width=8.5cm]{images/sfim_bad1/MPPI_CKF_16.png}}\hfil 

\subfigure[Radars move toward targets as closely as feasible.]{\includegraphics[width=8.5cm]{images/sfim1/MPPI_CKF_436.png}} \hfil 
\subfigure[Radars encircle targets, but the bottom most radar remains distant.]{\includegraphics[width=8.5cm]{images/sfim_bad1/MPPI_CKF_436.png}}\hfil  

\subfigure[Radars maintain circular formation with targets circle formation.]{\includegraphics[width=8.5cm]{images/sfim1/MPPI_CKF_668.png}} \hfil 
\subfigure[Radars encircle the targets, but bottom most radar moves away from targets.]{\includegraphics[width=8.5cm]{images/sfim_bad1/MPPI_CKF_668.png}}\hfil  

\subfigure[Radars maintain a circular formation within the circle of targets.]{\includegraphics[width=8.5cm]{images/sfim1/MPPI_CKF_1000.png}} \hfil 
\subfigure[Radars maintain encirclement formation around targets cricle]{\includegraphics[width=8.5cm]{images/sfim_bad1/MPPI_CKF_1000.png}}\hfil  

\caption{ \small 
The left column shows snapshots of target localization using a range measurement model with covariance dependent on radar-target distance \cite{godrich2010target}, while the right column depicts tracking with a range measurement model employing constant diagonal covariance \cite{bishop2010optimality}. In the first three rows, each subfigure's left panel shows a 3D projection onto 2D of continuous optimal radar placement at a specific time. The colored lines emanating from the radars depict the weighted MPPI-planned trajectories, with blue indicating better paths and red indicating worse ones. Dashed red and green circles mark the radar's (10 [m]) and the target's (125 [m]) collision avoidance boundaries, respectively, while blue dashed circles represent the targets' collision avoidance boundary based on the CKF position estimate. The radar's trajectory is the last 25 time steps. The right panel displays the log determinant of the FIM concerning the 2D target position for the specific time step, meshed over the free space area, and evaluated at each mesh point. }
\label{fig:noise_compare}
\end{figure*}


% The final row illustrates the RMSE over time, showing that the range measurement model with constant covariance exhibits greater performance fluctuations.
\begin{figure*}[h!]
    \centering
    \subfigure[C]{\includegraphics[width=8.5cm]{images/rmse_overlayed1.pdf}} \hfil 
    \subfigure[D]{\includegraphics[width=8.5cm]{images/rmse_overlayed_sfimbad.pdf}}\hfil  
    \caption{A closer look at the difference target localization errors between constant covariance and radar-based covariance. The average RMSE over the targets' true state versus the CKF predicted state over 250 MC trials. The lightly shaded region is the 80\% highest density interval (HDI) over 250 MC trials.}
    \label{fig:rmse_comparison1}
\end{figure*}

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.90\columnwidth]{images/rmse_mse_realization1.pdf}
    \caption{RMSE for single simulation realization in \cref{fig:noise_compare}}
    \label{fig:mse_compare1}
\end{figure}

\begin{figure}[h!]
    \centering
\includegraphics[width=0.95\columnwidth]{images/MPPI_CKF_3_4_stationary.jpg}
    \caption{A snapshot at time step 1000 depicts 3 stationary radars attempting to localize 4 dynamic targets, showcasing their failure to effectively track the targets.}
    \label{fig:stationary_failure}
\end{figure}

The integration of all the algorithms outlined thus far in \cref{sec:radar_signal_model,sec:process_modeling,sec:fim_definition,sec:mpc_objective} constitutes our enhanced continuous optimal radar placement pipeline, described in \cref{alg:contoptimalradar,fig:system_diagram}.

\RestyleAlgo{ruled}
\SetKwComment{Comment}{/* }{ */}

\begin{algorithm}[hbt!]
\label{alg:contoptimalradar}
\caption{Continuous Optimal Radar Placement}
\KwData{$\chi^{R_{1:N}}_0$}
\KwResult{$\hat{\chi}^{T_{1:M}}_{1:T},\chi^{R_{1:N}}_{1:T}$}
% $y \gets 1$\;
% $X \gets x$\;
% $N \gets n$\;
\For{$k=1:T$}{
 $\chi^{T_{1:M}}_{k+1}$ = TransitionFn$\left(\chi^{T_{1:M}}_{k}\right)$ \\
 $\hat{\chi}^{T_{1:M}}_{k+1}$ = CKF.predict$\left(\hat{\chi}^{T_{1:M}}_{k}\right)$ \\
  \If{$k\% T_{control}=0$}{
    $\hat{\chi}^{T_{1:M}}_{k+1:k+K} \gets$ CKF.propogate$\left(\hat{\chi}^{T_{1:M}}_{k+1}\right)$\;
    $\mathbf{u}_{k:k+K} \gets$ MPPI$\left(\hat{\chi}^{T_{1:M}}_{k+1:k+K},\chi^{R_{1:M}}_k,\right)$\;
    % cost = MPC$\left(\mathbf{u}_{k:k+K},\chi^{R_{1:N}}_k,\hat{\chi}^{T_{1:M}}_{k+1:k+K}\right)$
    % \Comment*[r]{This is a comment}
    $\mathbf{u}_{k:k+T_{control}}$ = repeat$\left(u_k, T_{control}\right)$ 
    % \Comment*[r]{\tiny due to the control update frequency being smaller than the CKF frequency}
  }
  $\chi^{R_{1:N}}_{k+1} \gets $ Actuate$\left(\chi^{R_{1:N}}_{k},\mathbf{u}_k\right)$ \;
  $\mathbf{z}^{R_{1:N}}_{k+1}$ = MeasureRange$\left(\chi^{T_{1:M}}_{k+1},\chi^{R_{1:N}}_{k+1}\right)$ \;
  $\hat{\chi}^{T_{1:M}}$ = CKF.update$\left(\chi_{k+1}^{R_{1:N}},\mathbf{z}^{R_{1:M}}_{k+1}\right)$ \;
}
\end{algorithm}

\vspace{-0.5cm}

==> methodology/methodology_draft3.tex <==
\section{Radar Signal Model}
\label{sec:radar_signal_model}
Following the approach in \cite{godrich2010target}, we assume there are $N$ radars transmitting orthogonal narrowband signals to track $M$ targets. In this setup, the received signal at radar $n$ for target $m$ is given by:
%
\begin{align}
    r^{nm}(t) &= \sum_{b=1}^N \zeta^{nm} e^{-j2\pi f_c \tau^{nm}} s^b(t-\tau^{nm}) + \epsilon_{a}^n(t), \label{eqn:return_signal} 
\end{align}
where the time delay is:
\begin{align}
    \tau^{nm} &= \frac{\lVert \chib^{R_n}_{xyz} - \chib^{T_m}_{xyz} \rVert  +  \lVert \chib^{R_b}_{xyz} - \chib^{T_m}_{xyz} \rVert} {c},
\end{align}
%
and the set of orthonormal lowpass equivalent signals $s(t)$ such that there is no signal interference when multiple radars transmit simultaneously.
The return signal noise $\epsilon_{a}(t)$ is circularly symmetric, zero-mean, complex Gaussian noise with autocorrelation function $\sigma_a^2 \delta (\tau)$. $\zeta$ is the complex amplitude of the return signal, where $|\zeta|^2$ is the radar power return specified by the radar equation \cite{barton2013radar}:
\begin{align}
    |\zeta|^2 = P_r = \frac{P_t \Lambda_t \Lambda_r \lambda^2 \Xi}{(4\pi)^3 \lVert \chib^{R}_{xyz} - \chib^{T}_{xyz} \rVert ^4 L}
\end{align}
The radar parameters specifying the received power $P_r$ $[W]$ at the radar include $P_t$ as the transmit power $[W]$, $\Lambda_t$ and $\Lambda_r$ as the transmit and receive gains, $L$ as the general loss factor, $\Xi$ as the radar cross section $[m^2]$, and $\lambda$ as the carrier frequency wavelength $[m]$.

It has been shown that the range measurement between radar $n$ and target $m$ approximately follows a Gaussian \gls{pdf} with variance parameterized by the radar-target geometry \cite{bishop2010optimality}.
\begin{align}
z^{nm} \sim  \mathcal{N}\left(2 \lVert \chib^{R_n}_{xyz} - \chib^{T_m}_{xyz} \rVert \; , \; \frac{c^2 \sigma_a^2}{8\pi^2 f_c^2 |\zeta^{nm}|^2} \right) \label{eqn:range_measurement}
\end{align}
We denote all the radar parameters, signal parameters, and noise parameters as a constant $\Gamma=\frac{c^2 \sigma_a^2 (4\pi)^3 L}{P_t \Lambda_t \Lambda_r \lambda ^2 \Xi 8\pi^2 f_c^2} $. For brevity, we define shorthand notation  as 
$h^{nm} = 2 \lVert \chib^{R_n}_{xyz} - \chib^{T_m}_{xyz} \rVert $ and $\sigma_z^{nm} = \Gamma \norm{\chib^{R_n}_{xyz} - \chib^{T_m}_{xyz}}^4 $. %\frac{c^2 \sigma_a^2}{8\pi^2 f_c^2 |\zeta^{nm}|^2}$.

Existing research has explored optimal radar placement when the covariance matrix of the range measurement depends on the radar-target geometry \cite{moreno2011optimal,yan2017exact,he2015generalized}, primarily focusing on stationary targets and radars. Given that the range measurement model relies on the positions of both the radars and targets, the next section describes the target and radar kinematic models. This will facilitate the definition of the targets' conditional transition probability in the targets' state space model.

\vspace{-1em}
\section{Process Model}
\label{sec:process_modeling}
We describe the kinematic model of a target to finalize the probabilistic state space model for the concatenated state of all the targets, encompassing both a conditional transition probability and the conditional measurement probability described in \ref{sec:radar_signal_model}.

\vspace{-1em}
\subsection{Target Kinematics: Constant Velocity Model}
The target kinematic model for a single target follows constant velocity motion with acceleration noise \cite{baisa2020derivation}, which specifies the single-target transition model:
\begin{align}
\chib^T_{k+1} &= A\chib_k^T + \epsilon_w \label{eqn:dynamics_single_target} 
\end{align}
where 
\begin{align}
    A_{\text{single}} &= \begin{bmatrix}
        1 & 0 & 0 & \Delta t & 0 & 0 \\ 
        0 & 1 & 0 & 0 & \Delta t & 0 \\ 
        0 & 0 & 1 & 0 & 0 & \Delta t \\ 
        0 & 0 & 0 & 1 & 0 & 0 \\
        0 & 0 & 0 & 0 & 1 & 0 \\
        0 & 0 & 0 & 0 & 0 & 1 \\
    \end{bmatrix} 
\end{align}
and $\epsilon_w$ is the acceleration noise which follows a zero  mean Gaussian \gls{pdf} with covariance
\begin{align}
         W_{\text{single}} &= \begin{bmatrix}
        \frac{\Delta t^4}{4} & 0 & 0 & \frac{\Delta t^3}{2} & 0 & 0 \\ 
        0 & \frac{\Delta t^4}{4} & 0 & 0 & \frac{\Delta t^3}{2} & 0 \\ 
        0 & 0 & \frac{\Delta t^4}{4} & 0 & 0 & \frac{\Delta t^3}{2}\\ 
        \frac{\Delta t^3}{2} & 0 & 0 & \Delta t^2 & 0 & 0 \\
        0 & \frac{\Delta t^3}{2} & 0 & 0 & \Delta t^2 & 0 \\
        0 & 0 & \frac{\Delta t^3}{2} & 0 & 0 & \Delta t^2\\
    \end{bmatrix} \cdot \sigma_W^2
\end{align}
$\sigma_W$ determines the degree of deviation of the dynamics from constant velocity, determined by the strength of the acceleration variance.
Thus, the targets' transition model (for all targets concatenated as a column vector) is:
\begin{align}
     \chib^{T_{1:M}}_{k+1} &= A \chib^{T_{1:M}}_k + \epsilon_{W} \label{eqn:transition_model} \\
    A &= \bm{I}_{M} \otimes A_{\text{single}} \quad W = \bm{I}_{M} \otimes W_{\text{single}} 
\end{align}
where $I_{M}\in \Re^{M\times M}$ is the identity matrix. Similarly, the measurements of all radar-target pairs may be concatenated to measurement measurement model of the targets' state-space equations (based on \cref{eqn:range_measurement}):
\begin{align}
\mathbf{z}^{T_{1:M}} &= \begin{bmatrix}
h^{11} & \ldots & h^{1M} \\
h^{21} & \ldots & h^{2M} \\
\vdots & \ddots & \vdots \\
h^{N1} & \ldots & h^{NM} \\
\end{bmatrix} +  \begin{bmatrix}
\sigma_z^{11} & \ldots & \sigma_z^{1M} \\
\sigma_z^{21}  & \ldots & \sigma_z^{2M}  \\
\vdots & \ddots & \vdots \\
\sigma_z^{NM} & \ldots & \sigma_z^{nM}  \\
\end{bmatrix} \odot \epsilon_\mathbf{z} \label{eqn:measurement_prob} \\
&= \mathbf{H(\chib^{T_{1:M}}_{xyz}}) + \Omega \odot \sigma_\mathbf{z}
\end{align}
where $\sigma_z^{nm}$ is the standard deviation of the range measurement for radar $n$ and target $m$, as defined by the variance in \cref{eqn:range_measurement}, while $\sigma_z$ is standard normal Gaussian \gls{pdf}. Therefore the final state-space equations for the targets is shown in \cref{eqn:state_space_meas,eqn:state_space_tran}:
\begin{align}
     \chib^{T_{1:M}}_{k+1} &= A\chib^{T_{1:M}}_k + \epsilon_{W} \label{eqn:state_space_tran} \\
    \mathbf{z}^{T_{1:M}}_{k+1} &= \mathbf{H}\left((\chib^{T_{1:M}}_{xyz})_{k+1}\right) + \Omega \odot \sigma_\mathbf{z} \label{eqn:state_space_meas} 
\end{align}
Given our focus on dynamic targets and dynamic radars, it's essential to outline a basic kinematic model where the radar position is determined by control inputs and adheres to specific control and dynamic constraints. Thus, we next define the second-order unicycle kinematic model for the radars.

\vspace{-1em}
\subsection{Radar Kinematics: Second-Order Unicycle Model}
Each radar follows the second-order unicycle model. We use the Euler discretization of the unicycle continuous dynamic model with heading acceleration and angular acceleration control inputs $u = [u_{a},u_{\dot{\omega}}]^T$ to define the discrete time kinematic model:

% x_{k+1} &= x_{k} + \dot{x}_k \cos{\theta_k} \Delta t + \frac{1}{2} (u_{a})_k \cos{\theta_k} \Delta t^2  \\
% y_{k+1} &= y_{k} + \dot{y}_k \sin{\theta_k} \Delta t + \frac{1}{2} 
% (u_{a})_k \sin{\theta_k} \Delta t^2 \\
% z_{k+1} &= z_{k} \\
% \theta_{k+1} &= \theta_{k} + \omega_k \Delta t + \frac{1}{2} u_{\dot{\omega}_k} \Delta t^2 \\
% \vvec_{k+1} &= \vvec_k + (u_{a})_k \Delta t \\
% \omega_{k+1} &= \omega_{k} + (u_{\dot{\omega}})_k \Delta t \\

\begin{align}
    \chib^{R}_{k+1} &= \chib^{R}_k + G_k(\chib^{R}_k,u_k) \label{eqn:radar_kinematics}
\end{align}
with control, velocity, and angular velocity limits,
\begin{equation}
\begin{aligned}
\begin{split}
\underbar{$u$}_a \leq u_{a_k} &\leq \bar{u}_a \; \forall k \\
\underbar{$u$}_{\dot{\omega}} \leq u_{\dot{\omega}_k} &\leq \bar{u}_{\dot{\omega}} \; \forall k  \\
\end{split} \quad
\begin{split}
\underbar{$v$} \leq v_k &\leq \bar{v} \; \forall k \\
\underbar{$\omega$} \leq \omega_k &\leq \bar{ \omega } \; \forall k. 
\end{split}
\end{aligned}
\label{eqn:radar_kinematics_constrained}
\end{equation}
With the radars' positions defined relative to control inputs, the following section outlines the derivation of the \glspl{fim} with respect to the targets' positions. This is based on the radar-target measurement model outlined in  \cref{eqn:range_measurement,eqn:measurement_prob}, and the radars' positions parameterized by \cref{eqn:radar_kinematics,eqn:radar_kinematics_constrained}.

\vspace{-1em}
\section{Fisher Information Matrix}
\label{sec:fim_definition}

The \gls{sfim} measures the amount of information that an observable random variable $z$ (range measurements) carries about an unknown parameter $\theta$ (targets' states) \cite{tichavsky1998posterior,kay1993fundamentals}:

\begin{align}
    \Jb_D(\theta) = E\left[\left( \nabla_{\theta} \log f\left(z|\theta \right) \right) \left( \nabla_{\theta} \log f\left(z|\theta \right) \right)^T\right]
\end{align}
Under the assumption of independence, the range measurements likelihood in \cref{eqn:measurement_prob} is represented as:
\begin{align}
    f\left(\mathbf{z}^{T_{1:M}}|\chib^{T_{1:M}}_{xyz} ; \chib^{R_{1:N}}_{xyz} \right) &= \prod_{n=1}^{N} \prod_{m=1}^{M} f(z^{nm} | \chib^{T_m}_{xyz} ; \chib^{R_n}_{xyz})
\end{align}
Given that the measurement is a Gaussian \gls{pdf}, with the mean and covariance parameterized by the targets' positions, and that information of measurements is additive by the independence assumption, we use the derivation of general Gaussian \gls{fim} \cite{kay1993statistical} to calculate the \gls{sfim} for a multiple targets' positions with multiple radars:
\begin{align}
    J(\chib^{T_m}_{xyz};\chib^{R_n}_{xyz}) &= (\chib^{T_m}_{xyz} - \chib^{R_n}_{xyz})(\chib^{T_m}_{xyz} - \chib^{R_n}_{xyz})^T \times \nonumber \\
    &\left( \frac{4}{K \lVert\chib^{R}_{xyz} - \chib^{T}_{xyz} \rVert^6} + \frac{8}{\lVert \chib^{R}_{xyz} - \chib^{T}_{xyz} \rVert^4} \right) \label{eqn:fim_single_radar_single_target} \\
    J(\chib^{T_m}_{xyz};\chib^{R_{1:N}}_{xyz}) &= \sum_{n=1}^N J(\chib^{T_m}_{xyz} ; \chib^{R_n}_{xyz})     \label{eqn:fim_multi_radar_single_target} 
\end{align}
\vspace{-2em}
\begin{align}
    &J(\chib^{T_{1:m}}_{xyz};\chib^{R_{1:n}}_{xyz}) = \nonumber \\
        &\begin{bmatrix}
        J(\chib^{T_{1}}_{xyz};\chib^{R_{1:N}}_{xyz}) & \!\! 0 & \!\!\ldots & \!\!0 \\
        0 & \!\! J(\chib^{T_{2}}_{xyz};\chib^{R_{1:N}}_{xyz}) & \!\! \ldots & \!\! 0 \\
        \vdots & \!\! \vdots & \!\! \ddots & \!\! \vdots \\
        0 & \!\! 0 & \!\! \ldots & \!\! J(\chib^{T_{M}}_{xyz};\chib^{R_{1:N}}_{xyz})
    \end{bmatrix} \label{eqn:fim_multi_radar_multi_target}
\end{align}
Equation \cref{eqn:fim_single_radar_single_target} is the \gls{sfim} of a single target position parameterized by a single radar and \cref{eqn:fim_multi_radar_single_target} is the \gls{sfim} of a single target positions parameterized by multiple radars.

When there is prior knowledge about the dynamics of the target state (\cref{eqn:dynamics_single_target}), then this information may be incorporated into the \gls{sfim} to form the \gls{pfim}:
\begin{align}
    \Jb = \Jb_D + \Jb_P \\
    \Jb_P = E[\Delta_{\chib^T}^{\chib^T} \log f(\chib^T)] \label{eqn:pfim_single}
\end{align}
Here, $\Jb_D$ represents the information about the unknown target state obtained from the data, while $\Jb_P$ reflects the information about the unknown target state based on prior assumptions. Now, considering that the targets' state includes velocity, we update \cref{eqn:fim_multi_radar_multi_target} to be $\Jb_D$ for the \gls{pfim}, with the block matrices as:
\begin{align}
&J(\chib^{T_n};\chib^{R_{1:N}}_{xyz}) =  \begin{bmatrix}
    J(\chib^{T_n}_{xyz};\chib^{R_{1:N}}_{xyz}) & 0 \\
    0 & 0
\end{bmatrix}  \label{eqn:fim_multi_radar_multi_target_velocity} 
\end{align}

For discrete time filtering systems, such as \cref{eqn:state_space_meas,eqn:state_space_tran}, the
\cref{eqn:pfim_single} is recursively computed at time $k+1$ from time step $k$ using the famous recursion updates in \cite{tichavsky1998posterior}. The recursion equations are written as 
\begin{align}
    &\Jb_{k+1} (\chib^{T_{1:M}}_{k+1}) = \Db_k^{22} - \Db_k^{21} (\Jb_k + \Db_k^{11})^{-1} \Db_k^{12} \label{eqn:pfim_recursion}
\end{align}
where
\begin{align}
    &\Db_k^{11} = E[-\Delta_{\chib^{T_{1:M}}_k}^{\chib^{T_{1:M}}_k} \log p(\chib^{T_{1:M}}_{k+1} | \chib^{T_{1:M}}_k)]  \\
    &\Db_k^{12} = E[-\Delta_{\chib^{T_{1:M}}_k}^{\chib^{T_{1:M}}_{k+1}} \log p(\chib_{k+1} | \chib_k)] = [\Db_k^{21}]^T \\
    &\Db_k^{22} = E\left[-\Delta_{\chib^{T_{1:M}}_{k+1}}^{\chib^{T_{1:M}}_{k+1}} \log p(\chib^{T_{1:M}}_{k+1} | \chib^{T_{1:M}}_{k}) \right] + \nonumber \\
    & \qquad E\left[-\Delta_{\chib^{T_{1:M}}_{k+1}}^{\chib^{T_{1:M}}_{k+1}} \log p(z_{k+1} | \chib^{T_{1:M}}_{k+1}) \right] 
\end{align}
Each $D$ term in equation \cref{eqn:pfim_recursion} is (\gls{pdf} regularity assumptions) as 
\begin{align}
    &\Db_k^{11} =\Ab^T \Wb^{-1} \Ab  \label{eqn:d11}\\
    &\Db_k^{12} = - \Ab^T \Wb^{-1} \label{eqn:d12} \\
    &\Db_k^{22} =  \Wb^{-1} + E_{f(\chib^{T_{1:M}}_{1:k+1})} \left[-\Jb_{\Db_k}(\chib^{T_{1:M}}_{k+1})) \right] \label{eqn:d22}
\end{align}
where due to the Markov assumption on the transition model in the targets' state space equation (\cref{eqn:transition_model}), the joint \gls{pdf} $f(\chib^{T_{1:M}}_{1:k})$ is simplified as
\begin{align}
    f(\chib^{T_{1:M}}_{1:k}) = f(\chib^{T_{1:M}}_{0}) \prod_{t=1}^{k+1} f(\chib^{T_{1:M}}_{t} | \chib^{T_{1:M}}_{t-1}) \label{eqn:markov_simplified}
\end{align}
After substituting equations \cref{eqn:d11,eqn:d12,eqn:d22} into \cref{eqn:pfim_recursion}, and leveraging the Woodbury matrix identity \cite{bishop2006pattern}, we arrive at  \cite{simplifed_pfim_recursion}:
\begin{align}
    \Jb_{k+1} (\chib^{T_{1:M}}_{k+1}) &= (W + A^T \Jb_k^{-1} A)^{-1} + \notag \\ & \quad  \quad E_{f(\chib^{T_{1:M}}_{1:k+1})} \left[-\Jb_{\Db_k}(\chib^{T_{1:M}}_{k+1})) \right] \label{eqn:pfim_simplified}
\end{align}
\cref{eqn:pfim_simplified} is preferred over \cref{eqn:pfim_recursion} for numerical stability. This preference arises because it avoids the inversion of the $W$ matrix, which can be close to singular in cases where the conditional transition PDF is described by constant velocity models.

To compute the expectation over the target state for \cref{eqn:d22}, as well as objective terms involving \cref{eqn:fim_multi_radar_multi_target} or any other objective term in the \gls{mpc} objective that involves the targets' states, we employ the \gls{ckf} to describe \cref{eqn:markov_simplified}.

\glspl{ckf} efficiently leverage third-order spherical cubature integration into both the prediction and correction steps of an additive Gaussian noise Kalman filter \cite{sarkka2023bayesian}. To compute the expectations described in the previous paragraph, we propagate the sigma points of the \gls{ckf} multiple time steps into the future, employing a number of sigma points equal to twice the dimension of the state variable. Compared to a \gls{pf} \cite{sarkka2023bayesian}, the \gls{ckf} has lower computational complexity, as the number of evaluation points scales linearly with the state size, while the number of particles in a \gls{pf} may substantially increase.

With our current formulations in \cref{sec:radar_signal_model,sec:process_modeling,sec:fim_definition}, we formulate a discrete-time finite-horizon \gls{mpc} objective  using dynamic, control, and mission-aware constraints.

\vspace{-1em}
\section{Model Predictive Controller Objective}
\label{sec:mpc_objective}
\gls{mpc} is an optimal control technique that determines the control actuation minimizing a cost function for a constrained dynamical system over a finite, receding horizon \cite{morari1999model,khaled2018practical}. At each time step of the receding horizon objective, we enforce minimum distances between radars and targets to prevent potential destruction by adversaries using soft penalties. Similarly, we ensure safe separation distances between mobile radars to prevent collisions. Additionally, we incorporate the radar's acceleration, angular acceleration, angular speed, and heading velocity constraints as described in \cref{eqn:radar_kinematics_constrained} into the dynamic equation using clipping functions. Finally, we directly integrate the radar's dynamic equation (\cref{eqn:radar_kinematics_constrained}) into the objective using direct shooting \cite{directshooting}.

As a result, converting hard constraints to soft/implicit constraints results in an unconstrained, discontinuous, and non-differentiable optimization formulation. Lastly, we incorporate the uncertainty of the targets' state by taking expectation of the \gls{mpc} objective function with respect to the \gls{ckf} estimator of the targets' state:
{\hspace{-5cm}
\begin{align}
    &S(\uvec_{k:k+K+1} ; \chib^{T_{1:M}}_{k:k+K+1}) \!=\!  E_{\tilde{f}} \bigr[S_{traj}(\uvec_{k:k+K+1} ; \chib^{T_{1:M}}_{k:k+K+1})  \notag \\
    & \quad \quad \quad  \quad \quad \quad \quad  + \alpha_1 S_{R2R}(\uvec_{k:k+K}) \notag \\
    & \quad \quad \quad  \quad \quad \quad \quad + \alpha_2 S_{R2T}(\uvec_{k:k+K} ; \chib^{T_{1:M}}_{k:k+K}) \bigr] \label{eqn:mpc_obj_unconstrained}  \\
    &\text{where } \notag\\
    & S_{traj}\left(\chib^{R_{1:N}}_{k:k+K+1} ; \chib^{T_{1:M}}_{k:k+K+1}\right) = \notag \\
    &\quad \sum_{t=k}^{k+K+1} \gamma^{t-k} \log \det \left(J(\chib_{t}^{T_{1:M}} ; \chib_{t}^{R_{1:M}} \right)  \notag   \\
    & S_{R2T}(\uvec_{k:k+K+1} \!) \! = \notag \\
    &\quad \; \; \!\! \sum_{t=k}^{k+K+1} \!\! \gamma^{t-k} \!\! \sum_{m=1}^M \! \sum_{n=1}^N \! \mathbf{1} \! \left( \lVert \chib_t^{T_n} \! + \! \chib_t^{R_m}(\uvec_{t})  \rVert \! \leq \! R_{R2T} \! \right) \notag \\
    & S_{R2R}(\uvec_{k:k+K+1}) = \notag \\
    & \quad \; \sum_{t=k}^{k+K+1} \gamma^{t-k} \!\!\!\!\!\! \sum_{\{i<j: i,j \in M\}} \!\!\!\!\!\! \mathbf{1} \left( \lVert \chib_t^{R_i}(\uvec_{t}) - \chib_t^{R_j}(\uvec_{t})  \rVert \leq R_{R2R} \right) 
\end{align} 
where $\alpha_1,\alpha_2$ are hyper parameters that determine how much to penalize the radars for violating the soft constraints $S_{R2R},S_{R2T}$ respectively, $\gamma$ is the discount factor, and $K$ is the horizon length. The \gls{ckf} estimator \gls{pdf} on the targets' state over the horizon is
\begin{align}
\tilde{f}(\chib_{k:k+K+1}^{T_{1:M}}) = f_{ckf}(\chib^{T_{1:M}}_{k}|\mathbf{z}_{1:k-1}) \! \prod_{t=k+1}^{k+K+1} \! f(\chib^{T_{1:M}}_{t} | \chib^{T_{1:M}}_{t-1})    
\end{align}
}


This \gls{mpc} problem requires an efficient solver that can handle highly nonlinear, discontinuous, and non-differentiable functions. Therefore, we employ a sampling-based strategy, \gls{mppi} \cite{williams2018information}, as discussed in the following section.

\vspace{-1em}
\subsection{Model Predictive Path Integral}
\gls{mppi} is a sampling-based \gls{mpc} algorithm designed for optimizing nonlinear stochastic systems subject to complex cost functions in real time \cite{7487277}. The assumption of \gls{mppi} is the control input is random and distributed as Gaussian random vector $\vvec \sim N(\uvec,\bm{\Sigma})$. Due to the stochasticity of the control input, rather than solving for a deterministic optimal control input we solve for an optimal control \gls{pdf} $Q^*$ \cite{theodorou2010generalized}: 
\begin{align}
    Q^* = \frac{1}{\eta} \exp\left(-\frac{1}{b}S(\vvec_{k:k+K+1}) \right) P(\vvec_{k:k+K+1})
\end{align}
where $P(\cdot)$ is the \gls{pdf} of an control input sequence in an uncontrolled system ($\uvec_{k:k+K+1} = 0)$, $b$ is the temperature of the distribution, and $\eta$ is the evidence.
However, the optimal control \gls{pdf} likely does not possess an analytical form. Therefore, by minimizing the \gls{kbl} betwewen $Q^*$ and a variational Gaussian \gls{pdf} $Q$ parameterized by $u,\Sigma$ \cite{williams2018information} with respect to $u$ gives the optimal control at $k$ as \cite{williams2018information} 
\begin{align}
    \uvec^*_k = \int q^*(\bigvvec) \vvec_k d\bigvvec \label{eqn:optimal_control_mppi}
\end{align}

Since we cannot express $Q^*$ analytically in \cref{eqn:optimal_control_mppi}, we leverage \gls{ais} to approximate the expectation as follows \cite{asmar2023model,williams2018information}: 
\begin{enumerate}
    \item sample control trajectories $\vvec_{k:k+K+1}^{(i)}$ from distribution $Q$ with mean $\uvec_{k:k+K+1}$ and covariance $\Sigma$
    \item evaluate the objective function for each control trajectory sample $S(\vvec_{k:k+K+1}^{(i)})$
    \item compute the importance sampling corrective weights for each sample $\tilde{w}^{(i)} \propto S(\vvec^{(i)})$
    \item adapt the mean and covariance of the \gls{pdf} $Q$ 
    \item repeat steps 1-4
\end{enumerate}

Due to the high dimensionality of the targets' control input over a horizon and the limited number of samples in \gls{mppi}, the sample covariance matrix for control inputs can overfit, leading to inaccurate variances \cite{theiler2012incredible}. This often results in poor control inputs from the proposal distribution of \gls{mppi}. To address this, we adopt the \gls{lw} for \gls{ais}, which approximates \gls{oas} shrinkage and helps mitigate overfitting, following the method described in \cite{asmar2023model}.

\begin{figure*}[h!]

\centering
\subfigure[Proposed approach: Each radar moves towards the targets.]{\includegraphics[width=8.5cm]{images/sfim1/MPPI_CKF_16.png}}\hfil
\subfigure[\cite{hung2020range,bishop2010optimality,crasta2018multiple} range model: The upper right radar moves away from targets]{\includegraphics[width=8.5cm]{images/sfim_bad1/MPPI_CKF_16.png}}\hfil 
\vspace{-.5em}
\subfigure[Radars move toward targets as closely as feasible.]{\includegraphics[width=8.5cm]{images/sfim1/MPPI_CKF_436.png}} \hfil 
\subfigure[Radars encircle targets, but the bottom most radar remains distant.]{\includegraphics[width=8.5cm]{images/sfim_bad1/MPPI_CKF_436.png}}\hfil  
\vspace{-.5em}
\subfigure[Radars maintain circular formation with targets circle formation.]{\includegraphics[width=8.5cm]{images/sfim1/MPPI_CKF_668.png}} \hfil 
\subfigure[Radars encircle the targets, but bottom most radar moves away from targets.]{\includegraphics[width=8.5cm]{images/sfim_bad1/MPPI_CKF_668.png}}\hfil  
\vspace{-.5em}
\subfigure[Radars maintain a circular formation within the circle of targets.]{\includegraphics[width=8.5cm]{images/sfim1/MPPI_CKF_1000.png}} \hfil 
\subfigure[Radars maintain encirclement formation around targets cricle]{\includegraphics[width=8.5cm]{images/sfim_bad1/MPPI_CKF_1000.png}}\hfil  
\vspace{-.5em}
\caption{ \small 
The left column shows snapshots of target localization using a range measurement model with covariance dependent on radar-target distance \cite{godrich2010target}, while the right column depicts tracking with a range measurement model employing constant diagonal covariance \cite{bishop2010optimality}. In the first three rows, each subfigure's left panel shows the 3D projection onto 2D of continuously optimizing radar placement at a specific time. The colored lines emanating from the radars depict the weighted MPPI-planned trajectories, with blue indicating better paths and red indicating worse ones. Dashed red and green circles mark the radar's (10 [m]) and the target's (125 [m]) collision avoidance boundaries, respectively, while blue dashed circles represent the targets' collision avoidance boundary based on the CKF position estimate. The radar's trajectory is the last 25 time steps. The right panel displays the log determinant of the FIM (for the ddr measurement model) concerning the 2D target position for the specific time step, meshed over the free space area, and evaluated at each mesh point. }
\label{fig:noise_compare}
\end{figure*}

\RestyleAlgo{ruled}
\SetKwComment{Comment}{/* }{ */}

\begin{algorithm}[hbt!]
\caption{Continuous Optimal Radar Placement}\label{alg:contoptimalradar}
\KwData{$\chib^{R_{1:N}}_0$}
\KwResult{$\hat{\chib}^{T_{1:M}}_{1:T},\chib^{R_{1:N}}_{1:T}$}
% $y \gets 1$\;
% $X \gets x$\;
% $N \gets n$\;
\For{$k=1:T$}{
 $\chib^{T_{1:M}}_{k+1}$ = TransitionFn$\left(\chib^{T_{1:M}}_{k}\right)$ \\
 $\hat{\chib}^{T_{1:M}}_{k+1}$ = CKF.predict$\left(\hat{\chib}^{T_{1:M}}_{k}\right)$ \\
  \If{$k\% T_{control}=0$}{
    $\hat{\chib}^{T_{1:M}}_{k+1:k+K+1} \gets$ CKF.propogate$\left(\hat{\chib}^{T_{1:M}}_{k+1}\right)$\;
    $\mathbf{u}_{k:k+K+1} \gets$ MPPI$\left(\hat{\chib}^{T_{1:M}}_{k+1:k+K+1},\chib^{R_{1:M}}_k,\right)$\;
    % cost = MPC$\left(\mathbf{u}_{k:k+K+1},\chib^{R_{1:N}}_k,\hat{\chib}^{T_{1:M}}_{k+1:k+K+1}\right)$
    % \Comment*[r]{This is a comment}
    % $\mathbf{u}_{k:k+T_{control}}$ = repeat$\left(\uvec_k, T_{control}\right)$ 
    % \Comment*[r]{\tiny due to the control update frequency being smaller than the CKF frequency}
  }
  $\chib^{R_{1:N}}_{k+1} \gets $ Actuate$\left(\chib^{R_{1:N}}_{k},\mathbf{u}_k\right)$ \;
  $\mathbf{z}^{R_{1:N}}_{k+1}$ = MeasureFn$\left(\chib^{T_{1:M}}_{k+1},\chib^{R_{1:N}}_{k+1}\right)$ \;
  $\hat{\chib}^{T_{1:M}}$ = CKF.update$\left(\chib_{k+1}^{R_{1:N}},\mathbf{z}^{R_{1:N}}_{k+1}\right)$ \;
}
\end{algorithm}

The integration of the algorithms outlined in \cref{sec:radar_signal_model,sec:process_modeling,sec:fim_definition,sec:mpc_objective} forms the enhanced continuous optimal radar placement pipeline, described in Algorithm 1. This pipeline includes two key enhancements: an improved range measurement model, which significantly impacts the \gls{fim}, and a flexible and computationally efficient \gls{mpc} objective optimizer using \gls{mppi}.

==> relatedwork/relatedword_draft1.tex <==
\section{Related Work}
\label{sec:related_works}
\begin{enumerate}
    \item \textcolor{red}{Static target localization}
    \item \textcolor{red}{Dynamic target localization}
    \item \textcolor{red}{Multi-agent coordination},
    \item \textcolor{red}{\gls{mpc} optimizers}
\end{enumerate}

\textcolor{red}{Static Radar Placement - Static Target} 


Because various forms of the \gls{fim} establish a fundamental estimation limit for unbiased estimators, and information is additive under the assumption of independent measurements, numerous authors construct a D/A-optimality objective as a function of the \gls{fim} parameterized by the sensors position and the estimated target(s) position.
\cite{wireless_network_pos}

Many works on optimal radar placement use range measurements assumed to be coming from Gaussian distributions to construct the \gls{fim}, where the covariance is a function of the distance between the sensor and the target \cite{jiang2015optimal,bishop2010optimality,moreno2011optimal,godrich2010target,hu2017cramer,yan2017exact}. 
In cases where the range measurement covariance is independent of the sensor-target distance, studies such as \cite{jiang2015optimal,bishop2010optimality} reveal that the optimal sensor placement is determined solely by the angle between the sensor and the target, neglecting the distance between sensor and target. However, this approach is unrealistic because it overlooks signal path attenuation, which should ideally result in higher information gain for a sensor when it is closer to the target. To compensate for this, \cite{moreno2011optimal,jourdan2008optimal} employ a heuristic assumption made regarding the covariance, which combines a diagonal covariance matrix with another diagonal matrix representing the range between the sensors and the target. Yet, signal processing fundamentals offer even more realistic range measurement distributions. In \cite{godrich2010target,yan2017exact}, the covariance, proportional to the return radar power, is derived from optimizing the time delay of the Taylor series expansion of a match filter for a Narrowband return signal undergoing attenuation and passing through an \gls{awgn} channel. We use the signal processing fundamentals for a range measurement density following \cite{godrich2010target}. Despite the more realistic range measurement distribution, most of these works focus on static-sensor-static-target or static-sensor-dynamic-target scenarios. 

The works which focus on dynamic-sensor-dynamic target scenarios typically employ an \gls{mpc} objective by assuming the instantaneous cost is the the D/A-optimality of the \gls{fim} (or other information based metrics) \cite{hung2020range,crasta2018multiple,cai2021non,celeste2014optimal} which may be efficiently computed for discrete time nonlinear filtering via recursive equations \cite{tichavsky1998posterior}. \cite{crasta2018multiple,hung2020range} utilize multiple autonomous surface vehicle motion planning for cooperate range-based underwater target localization. However, the range measurement distribution assumes a constant diagonal covariance matrix which is not a function of range, and furthermore assume the target dynamic model covariance is 0. \cite{cai2021non}. \cite{cai2021non} minimizing the mutual information gain between the predict and the update steps of an Kalman Filter, and model the noise covariance of the measuremennt based on the robot's state.

==> relatedwork/relatedwork_draft2.tex <==
\section{Related Work}
\label{sec:related_works}


We will focus on the literature that utilizes the \gls{fim} of the range measure(s) likelihood for optimal trajectory generation of the sensor(s), with the likelihood parameterized by the target position(s). Various forms of the \gls{fim} establish a fundamental estimation limit for unbiased estimators, and information is additive under the assumption of independent sensor measurements. Therefore, numerous authors construct a D/A-optimality objective \cite{jones2021optimal} as a function of the \gls{fim} parameterized by the sensor position(s) and estimated target(s) position \cite{wireless_network_pos}. Since the \gls{pcrlb}, which is the inverse of the \gls{pfim}, evaluates estimator variance, and considering the bias-variance decomposition of mean squared error \cite{bishop2006pattern}, minimizing the mean squared error of an estimator is directly related to optimizing this D/A-optimality objective of the \gls{fim} matrix. The literature on optimal radar placement using the \gls{fim} of the sensor measurement likelihood for optimizing the sensor placement may be divided into two categories: static-sensor(s) versus dynamic-sensor(s)

We define static sensors as sensors that have no dynamic model or control input. When optimizing for the optimal placement of static sensors, this would be the positions of the sensors if you could magically place them in position instantaneously. Many works on optimal radar placement use range measurements assumed to be coming from Gaussian distributions to construct the \gls{fim}, where the covariance may or may  not be 
a function of the sensor(s)-target(s) distance \cite{jiang2015optimal,bishop2010optimality,moreno2011optimal,godrich2010target,hu2017cramer,yan2017exact}. 

In cases where the range measurement covariance is independent of the sensor-target distance, studies such as \cite{jiang2015optimal,bishop2010optimality} reveal that the optimal sensor placement is determined solely by the angle between the sensor and the target, neglecting the distance between sensor and target. However, this approach is unrealistic because it overlooks signal path attenuation, which should ideally result in higher information gain for a sensor when it is closer to the target. 

To compensate for this, \cite{moreno2011optimal,jourdan2008optimal} employ a heuristic assumption made regarding the covariance, which combines a diagonal covariance matrix with another diagonal matrix representing the range between the sensors and the target. Yet, signal processing fundamentals offer even more realistic range measurement distributions. In \cite{godrich2010target,yan2017exact}, the covariance, proportional to the return radar power, is derived from optimizing the time delay of the Taylor series expansion of a match filter for a Narrowband return signal undergoing attenuation and passing through an \gls{awgn} channel. We use the signal processing fundamentals for a range measurement density following \cite{godrich2010target}.
In practice, radars cannot simply "appear" at the optimal location; they require constrained dynamics and path planning. Additionally, dynamic sensors are necessary for dynamic targets, as the optimal radar configuration at one time step may no longer be optimal at the next time step.

Historically, two main approaches have been used for optimal radar placement in target localization of dynamic targets: 1) moving the radars to track dynamic targets while maintaining an optimal radar-target localization geometry \cite{martinez2006optimal,kumar2021recent}, and 2) "spraying" radars over a large area to ensure high spatial coverage and multiplicity, then selecting which radars to employ for sensing \cite{zhao2002information}. This paper primarily focuses on approach 1. 

We define dynamic sensors as sensors that possess the capability to adjust their positions or trajectories over time in response to changing environmental conditions or target dynamics. Consequentially, rather than directly optimizing the radar's position at a specific time step, as in the static-sensor formulation, the optimal radar trajectory is indirectly determined by optimizing the control inputs to the radar kinematic model by the method of direct shooting \cite{directshooting}. %\cite{martinez2006optimal,kumar2021recent}. 

% integrating the \gls{pcrlb}/\gls{pfim} in the instantaneous cost function.

The finite horizon \gls{mpc} objective may be computed efficiently by recursively computing the \gls{pcrlb} for discrete-time nonlinear filtering \cite{tichavsky1998posterior}. Several works on cooperative range-based underwater target localization with multiple autonomous surface vehicles utilize the aforementioned technique, while considering constraints such as distances between targets and sensors \cite{crasta2018multiple,hung2020range,sture2020trajectory}. However, the range measurement distribution assumes a constant diagonal covariance matrix that is not a function of range, and furthermore, they assume the target dynamic model covariance is 0.

\cite{he2020trajectory} employs a more complex measurement model that integrates traditional \gls{mtt} characteristics such as data association, track insertion, and track deletion using the \gls{jpdaf}. However, this work also assumes a constant diagonal covariance matrix for range and bearing measurements. Furthermore, the trajectory optimization only considers one time step ahead due to the (and therefore is not an \gls{mpc} objective) and only optimizes the sensor's heading angle.

Similar to information based \gls{mpc} objectives, \cite{cai2021non} minimizes the mutual information gain between the predict and the update steps of an linear Kalman Filter, while parameterizing the noise covariance of the measurement based on the robot's state. However, the measurement covariance grows linearly with the sensor-target distance, and is clipped at extremely small variance 0.01 meters, , which reflects in the experiments being confined to small square arenas of 40 meters to 60 meters.

==> relatedwork/relatedwork_draft3.tex <==
\section{Related Work}
\label{sec:related_works}


We explore literature using the \gls{fim} of range measurements' likelihood to optimize sensor trajectories, with the likelihood parameters as the target positions. Various forms of the \gls{fim} establish a fundamental estimation lower bound limit for the mean squared error covariance matrix \cite{bishop2006pattern}. Therefore, many authors construct an objective as the D/A-optimality \cite{jones2021optimal} of the \gls{pfim}, parameterized by sensor and estimated target positions \cite{wireless_network_pos}. We divide these works into two categories: those that consider static-sensors versus those that consider dynamic-sensors.

\vspace{-1em}
\subsection{Static Sensors}
Static sensors lack dynamic models or control inputs. Optimizing their placement involves determining where they would be positioned if placed instantaneously. Many studies on optimal radar placement use range measurements assumed to follow Gaussian distributions to construct the \gls{fim}, where the covariance may or may not vary with sensor-target distance \cite{jiang2015optimal,bishop2010optimality,moreno2011optimal,godrich2010target,hu2017cramer,yan2017exact}.

Several studies (e.g., \cite{jiang2015optimal,bishop2010optimality}) suggest that when the range measurement covariance is distance-independent, optimal sensor placement depends only on the angle between the sensor and the target. However, this approach overlooks the impact of signal path attenuation, which ideally results in higher information gain when the sensor is closer to the target.

To address this, \cite{moreno2011optimal,jourdan2008optimal} adopt a heuristic assumption concerning covariance, combining a constant diagonal matrix with another diagonal matrix which is a function of the range between sensors and targets. However, signal processing fundamentals provide more realistic range measurement distributions. We take a similar approach to \cite{godrich2010target,yan2017exact}, where the covariance, which scales with the return radar power, is determined by optimizing the Taylor series expansion of a match filter over time delay for a Narrowband return signal subject to attenuation and passing through an \gls{awgn} channel.
\vspace{-1em}
\subsection{Dynamic Sensors}
Practically, radars cannot simply ``appear'' at the optimal location; they require constrained dynamics and path planning. Moreover, dynamic sensors are essential to track dynamic targets, as the optimal radar configuration at one time step may not remain optimal at the next time step.

Historically, two main approaches have been used for optimal radar placement in target localization of dynamic targets: 1) moving the radars to track dynamic targets while maintaining an optimal radar-target localization geometry \cite{martinez2006optimal,kumar2021recent}, and 2) ``spraying'' radars over a large area to ensure high spatial coverage and multiplicity, then selecting which radars to employ for sensing \cite{zhao2002information}. This paper primarily focuses on the first approach, which is more appropriate given a limited number of radars.

Since the objective is a function of a finite horizon of time steps, many studies utilize an \gls{mpc} \cite{mpc_matlab} objective for optimizing the control inputs of mobile sensors \cite{khan2022design,uluskan2020noncausal,chu2020trajectory,sture2020trajectory,hung2020range}. Consequently, rather than directly optimizing the radar's position at a specific time step, as in the static-sensor formulation, the optimal radar trajectory is indirectly determined by optimizing the control inputs to the radar kinematic model using the method of direct shooting \cite{directshooting}.

% integrating the \gls{pcrlb}/\gls{pfim} in the instantaneous cost function.


The finite horizon \gls{mpc} objective, formulated in terms the \gls{pfim}, may be efficiently computed through recursive evaluation using discrete-time nonlinear filtering \cite{tichavsky1998posterior}. Several studies on cooperative range-based underwater target localization with multiple autonomous surface vehicles adopt this approach, while also considering constraints such as distances between targets and sensors \cite{crasta2018multiple,hung2020range,sture2020trajectory}. However, these methods often assume a constant diagonal covariance matrix for range measurements, irrespective of range, typically involve slow-moving sensors and targets, assume the target remains at a constant depth, and may assume a zero covariance for the target dynamic model.
Moreover, solving the resulting nonlinear optimization problems remains challenging, with several recent approaches leveraging \texttt{CasADi}~\cite{andersson2019casadi}.
% Moreover, these papers rely on the nonlinear optimization package \cite{andersson2019casadi} for solving the \gls{mpc}, which could impose limitations on the objective formulation and hinder real-time capabilities.

He et al \cite{he2020trajectory} employs a more complex measurement model which integrates \gls{mtt} characteristics such as data association, track insertion, and track deletion using the \gls{jpdaf}. However, this work assumes a constant diagonal covariance matrix for range and bearing measurements. Furthermore, the trajectory optimization only optimizes the sensor's heading angle one time step ahead due to the highly nonlinear objective function, potentially leading to myopic and suboptimal trajectories.

Similar to information based \gls{mpc} objectives like the D/A optimality of the \glspl{fim}, \cite{cai2021non} minimizes the mutual information gain between the predict and the update steps of a linear Kalman Filter, while parameterizing the noise covariance of the measurement based on the robot's state. However, the measurement covariance only scales linearly with the sensor-target distance and is clipped at an extremely small variance of 0.01 meters, restricting experiments to small square arenas of 40 to 60 meters.

Hence, the proposed approach aims to enhance target localization through continuously optimizing radar placement by integrating an improved range measurement model into the objective function. Additionally, we leverage \gls{mppi} control to increase flexibility in solving the \gls{mpc} objective over non-smooth and highly nonlinear objectives, enabling real-time control capabilities.
